Leveraging Memory Retrieval to Enhance LLM-based Generative Recommendation

Leveraging Large Language Models (LLMs) to harness user-item interaction histories for item generation has emerged as a promising paradigm in generative recommendation. However, the limited context window of LLMs often restricts them to focusing on recent user interactions only, leading to the neglect of long-term interests involved in the longer histories. To address this challenge, we propose a novel Automatic Memory-Retrieval framework (AutoMR), which is capable of storing long-term interests in the memory and extracting relevant information from it for next-item generation within LLMs. Extensive experimental results on two real-world datasets demonstrate the effectiveness of our proposed AutoMR framework in utilizing long-term interests for generative recommendation.

==> main/2_related_work.tex <==
\section{Related works}

Large language models (LLMs) have been widely applied in recommendation systems. Currently, researchers are focusing on leveraging the powerful generative capabilities of LLMs to enable generative recommendation. In this paradigm, LLMs directly generate text representations (e.g., item titles) of items that a user is likely to prefer, based on instructions constructed from the user's historical interactions. Generally, the items a user may prefer next are jointly determined by the user's short-term interests and long-term interests. A user's long-term interaction history contains abundant information about their long-term interests. A key research challenge in the context of generative recommendation with LLMs is how to effectively identify relevant long-term interests and integrate these with short-term interests. This has become a prominent topic in the field.

As a widely used technique in NLP, Retrieval-Augmented Generation (RAG) has been applied to recommendation systems powered by large language models (LLMs). Rella employs semantic similarity retrieval to search a memory bank composed of product titles interacted with by the user, using the target item’s title as a query. It then replaces the more temporally recent interacted items in the instruction with those that are semantically more relevant, determining whether the target item is worth recommending. However, there are two key limitations: (1) The concept of the target item exists only in discriminative recommendation scenarios; (2) In generative recommendation scenarios, where no explicit target item is available, the user's short-term interaction history must be used as a substitute for the target item in semantic retrieval. This substitution is unreliable, as the retrieved items often exhibit a significant gap from the long-term interests that the LLM truly requires. Consequently, the performance of the generative recommendation suffers considerable degradation.

We identify two core challenges in applying RAG to generative recommendation scenarios with LLMs:

1. \textbf{Retrieval Challenge}: For LLMs tasked with generating the next item, how can we define which long-term interests are relevant? Retrieval should identify long-term interests that, when combined with short-term interests, enhance the generative capability of the LLM. Simple retrieval approaches, such as semantic retrieval, may lead to conflicts between long- and short-term interests and hinder the LLM's understanding.

2. \textbf{Efficiency and Low Cost}: Retrieval models should be fast and cost-effective. Training a retrieval model for LLMs in an end-to-end manner is impractical. This approach involves injecting all historical data into the LLM and optimizing the retrieval model based on the LLM's loss. However, such a method is both computationally expensive and time-consuming during training and inference, making it unsuitable for efficient deployment.

To address this challenge, we propose \textbf{AutoMR}. AutoMR enhances a pre-trained LLM-based generative recommendation model (BigRec) by training an independent long-term interest retrieval model. The retrieved optimal long-term interests are incorporated into BigRec in the form of prefixes to improve its generative capability. Specifically, each block of the user's long-term interaction history (representing long-term interests) is inserted into BigRec as a prefix, and the resulting decrease in perplexity (PPL) is used to evaluate its relevance. Then, a retrieval model (an MLP) is trained by minimizing the distribution gap between the retrieval scores and the PPL reduction scores. This approach ensures that the most relevant long-term interests (those causing the greatest PPL reduction) are retrieved, enabling BigRec to better combine long- and short-term interests and predict the items the user is currently most interested in. Moreover, in generation stage, we observe that the LLM (BigRec) not only exhibits strong robustness in retrieving long-term interests, that is, It effectively prioritizes the most relevant information from both long- and short-term histories, but also can achieve a synergistic "1 + 1 > 2" effect.

In summary, our contributions are threefold:

1. To the best of our knowledge, this is the first work to explore the integration of users' long-term interest in generative recommendation scenarios.

2. We propose a novel method for defining users' relevant long-term interests by equipping a pre-trained LLM-based generative recommendation model with an independent long-term interest retrieval model.

3. We conduct extensive experiments on two widely used datasets, demonstrating that AutoMR significantly enhances the ability of large language models to incorporate long-term interests for generative recommendation.





==> main/backup/0_abs.tex <==
% Large Language Models (LLMs) have demonstrated significant potential in recommender systems, particularly in the paradigm of generative recommendation. Generally, in this paradigm, LLM generates textual representations of items that the user may prefer, based on instructions constructed from the user’s short-term historical interactions. However, effectively identifying relevant long-term interests and seamlessly integrating them with short-term interests to enhance recommendation performance remains a critical challenge. While the Retrieval-Augmented Generation (RAG) technique has been introduced in LLM-based recommendations, it often fails in generative recommendation scenarios due to its inability to reliably retrieve the long-term interests that LLMs truly require and to efficiently combine these with short-term interests. To address these limitations, we propose MemoRec, a novel framework that enhances a pre-trained LLM-based generative recommendation model (BigRec) by incorporating an independent long-term interest retrieval model. MemoRec identifies relevant long-term interests by evaluating their ability to reduce the LLM’s perplexity (PPL) and trains a lightweight retrieval model. Experimental results on two benchmark datasets demonstrate that MemoRec significantly improves the generative capability of LLMs by effectively integrating users’ long-term interests. Our work provides new insights into generative recommendation and highlights the importance of leveraging long-term interest modeling in LLM-based systems.
% , achieving a synergistic "1 + 1 > 2" effect

==> main/backup/1_intro.tex <==
\section{Introduction}
% 大语言模型已在推荐系统中得到广泛的应用。当前研究者们致力于利用大语言模型强大的生成能力做生成式推荐，即大语言模型基于由用户的历史交互构成的指令直接生成该用户接下来可能喜欢的商品文本表示，如商品标题。一般而言，用户接下来会喜欢的商品，通常由当下用户的短期兴趣，以及用户长期的兴趣共同决定。用户长期的交互历史中，包含有大量的用户长期兴趣。如何在大语言模型做生成式推荐的设定下，筛选出相关的长期兴趣以及有效融合筛选出的长期兴趣与短期兴趣的方法，是当前的热点话题。



Large language models (LLMs) have been widely applied in recommendation systems. Currently, researchers are focusing on leveraging the powerful generative capabilities of LLMs to enable generative recommendation. In this paradigm, LLMs directly generate text representations of items (e.g., item titles) that a user is likely to prefer, based on instructions constructed from the user's historical interactions. Due to disadvantages in terms of cost and performance, LLM-based generative models focus on leveraging short-term interactions to generate items, while neglecting the modeling of long-term interactions. Generally, the items a user may prefer next are jointly determined by the user's short-term interests and long-term interests. A user's long-term interaction history contains abundant information about their long-term interests. A key research challenge in the context of generative recommendation with LLMs is how to effectively identify relevant long-term interests and integrate these with short-term interests. This has become a prominent topic in the field.

% RAG作为NLP中广泛使用的技术已经被应用于大语言模型推荐系统上。Rella利用目标商品标题对由用户交互过的商品标题构成的记忆库进行语义相关性检索，将指令中原有的时间更近邻的已交互商品替换为语义相关性更强的已交互商品，判别目标商品是否值得被推荐。然而，1. 目标商品仅仅存在于判别式推荐场景中；2. 在生成式推荐场景下，我们只有通过用户的短期历史交互代替目标商品做语义检索，而该替代物对用户交互过商品的语义相关性检索是不可靠，即检索到的商品，与LLM真正需要的长期兴趣存在很大的差距，生成式推荐的性能严重下降。
As a widely used technique in NLP, Retrieval-Augmented Generation (RAG) has been applied to recommendation systems powered by LLMs. Rella employs semantic similarity retrieval to search a memory bank composed of item titles interacted with by the user, using the target item’s title as a query. It then replaces the more temporally recent interacted items in the instruction with those that are semantically more relevant, determining whether the target item is worth recommending. However, there are two key limitations: (1) The concept of the target item exists only in discriminative recommendation scenarios; (2) In generative recommendation scenarios, where no explicit target item is available, the user's short-term interaction history must be used as a substitute for the target item in semantic retrieval. This substitution is unreliable, as the retrieved items often exhibit a significant gap from the long-term interests that the LLM truly requires. Consequently, the performance of the generative recommendation suffers considerable degradation.

% 我们认为，RAG在大语言模型生成式推荐场景下的应用包含如下两个核心挑战：一是关于检索：对于LLM生成下一个商品，如何定义哪些长期历史兴趣是相关的。检索能够识别哪些长期兴趣和短期兴趣结合后会增强生成能力，简单的检索如语义检索会造成长短期兴趣的冲突和大语言模型的不理解。二是检索模型应该做到快速低成本。例如常见的通过端到端的方式训练检索模型是不现实的，该方法会将所有历史注入LLM中，训练出筛选有效检索模型，然而，这种方式训练和推理的成本高昂且耗时严重。
We identify two core challenges in applying RAG to generative recommendation scenarios with LLMs:

1. \textbf{Retrieval Challenge}: For LLMs tasked with generating the next item, how can we define which long-term interests are relevant? Retrieval should identify long-term interests that, when combined with short-term interests, enhance the generative capability of the LLM. Simple retrieval approaches, such as semantic retrieval, may lead to conflicts between long- and short-term interests and hinder the LLM's understanding.

2. \textbf{Efficiency and Low Cost}: Retrieval models should be fast and cost-effective. Training a retrieval model for LLM in an end-to-end manner is simply accessible but impractical. This approach involves injecting all historical data into the LLM and optimizing the retrieval model based on the LLM's loss. However, such a method is both computationally expensive and time-consuming during training and inference, making it unsuitable for efficient deployment.

% 为了达到这个目标，我们提出了MomeRec。MemoRec为一个已训练好的LLM生成式推荐模型（BigRec），训练了一个独立的长期兴趣检索模型，以prefix的方式将检索到的最优长期兴趣加入该BigRec中增强生成。首先将每条用户长期历史交互块（长期兴趣）的表示以prefix的方式插入到BigRec中，获得BigRec输出的ppl下降程度。其次，通过最小化检索分数的分布和ppl下降程度的分布来训练一个检索模型（MLP）。该方法定义的最相关的长期兴趣（ppl下降程度最大）有助于BigRec在融合长短期兴趣后，命中用户当前最感兴趣的商品。更多的，我们观察到，MemoRec不仅对长期历史的检索结果的优劣具有很强的鲁棒性，即能够在长短期历史中择优输出，更能够达到1+1>2的效果。
To address this challenge, we propose \textbf{MemoRec}. MemoRec enhances a pre-trained LLM-based generative recommendation model (BigRec) by training an independent long-term interest retrieval model. The retrieved optimal long-term interests are incorporated into BigRec in the form of prefixes to improve its generative capability. Specifically, each block of the user's long-term interaction (representing long-term interests) is inserted into BigRec as a prefix, and the resulting decrease in perplexity (PPL) is used to evaluate its relevance. Then, a retrieval model (an MLP) is trained by minimizing the distribution gap between the retrieval scores distribution and the PPL reduction distribution. This approach ensures that the most relevant long-term interests (those causing the greatest PPL reduction) are retrieved, enabling BigRec to better combine long- and short-term interests and predict the items the user is currently most interested in. In our experiments, Memorec demonstrated excellent capabilities in retrieving and leveraging long-term interests.
% Moreover, in generation stage, we observe that the LLM (BigRec) not only exhibits strong robustness in retrieving long-term interests, that is, it effectively prioritizes the most relevant information from both long- and short-term histories, but also can achieve a synergistic "1 + 1 > 2" effect.

% 总的来说，我们的贡献有三个方面：1. 在我们的知识范围内，这是第一个在生成式推荐场景下，探究结合用户长期历史做推荐的工作。2.提出了一种定义用户相关的长期兴趣的方法，为已训练好的LLM生成式推荐模型配备一个独立的长期兴趣检索模型，3. 我们在两个广泛使用的数据集上进行了大量实验，MemoRec提升了大模型结合长期兴趣做生成式推荐能力。
In summary, our contributions are threefold:

1. To the best of our knowledge, this is the first work to explore the integration of users' long-term interest in generative recommendation scenarios.

2. We propose a novel framework MemoRec for defining users' relevant long-term interests by equipping a pre-trained LLM-based generative recommendation model with an independent long-term interest retrieval model.

3. We conduct extensive experiments on two widely used datasets, demonstrating that MemoRec significantly enhances the ability of large language models to incorporate long-term interests for generative recommendation.





==> main/backup/1_intro_1217.tex <==
\section{Introduction}
% 大语言模型已在推荐系统中得到广泛的应用。当前研究者们致力于利用大语言模型强大的生成能力做生成式推荐，即大语言模型基于由用户的历史交互构成的指令直接生成该用户接下来可能喜欢的商品文本表示，如商品标题。一般而言，用户接下来会喜欢的商品，通常由当下用户的短期兴趣，以及用户长期的兴趣共同决定。用户长期的交互历史中，包含有大量的用户长期兴趣。如何在大语言模型做生成式推荐的设定下，筛选出相关的长期兴趣以及有效融合筛选出的长期兴趣与短期兴趣的方法，是当前的热点话题。

Recently, significant efforts~\cite{LLMRecSurvey} have been made to leverage the remarkable abilities of Large Language Models (LLMs) for recommendation tasks. Given LLMs' generative nature, a popular generative recommendation paradigm has emerged~\cite{bigrec,d3,genrec,lc-rec} --- teaching LLMs 
to leverage inputted historical interactions to
directly generate the next recommended item, without requiring predefined candidate items. In this paradigm, the inputted historical interactions provide user interest information, playing a pivotal role in determining the personalized item generation.
Due to computational costs and limited context windows, existing methods typically incorporate only the user's most recent interactions, overlooking longer histories. However, these extended histories encapsulate the user's long-term interests, a crucial aspect of user interests, neglecting which would inevitably lead to suboptimal performance.
% Due to the cost and limited context windows, existing work typically only incorporates the user's most recent interactions, neglecting longer histories. However, the long history captures the user's long-term interests, which is also an important aspect of recommendation.. Failing to model such information would undoubtedly result in suboptimal performance.
%%This paradigm shows the power of achieving promising results and exhibits some specific characteristics than other paradigms, e.g., global ranking abilities. 

% Large language models (LLMs) have been widely applied in recommendation systems. Currently, researchers are focusing on leveraging the powerful generative capabilities of LLMs to enable generative recommendation. In this paradigm, LLMs directly generate text representations of items (e.g., item titles) that a user is likely to prefer, based on instructions constructed from the user's historical interactions. Due to disadvantages in terms of cost and performance, LLM-based generative models focus on leveraging short-term interactions to generate items, while neglecting the modeling of long-term interactions. Generally, the items a user may prefer next are jointly determined by the user's short-term interests and long-term interests. A user's long-term interaction history contains abundant information about their long-term interests. A key research challenge in the context of generative recommendation with LLMs is how to effectively identify relevant long-term interests and integrate these with short-term interests. This has become a prominent topic in the field.

% RAG作为NLP中广泛使用的技术已经被应用于大语言模型推荐系统上。Rella利用目标商品标题对由用户交互过的商品标题构成的记忆库进行语义相关性检索，将指令中原有的时间更近邻的已交互商品替换为语义相关性更强的已交互商品，判别目标商品是否值得被推荐。然而，1. 目标商品仅仅存在于判别式推荐场景中；2. 在生成式推荐场景下，我们只有通过用户的短期历史交互代替目标商品做语义检索，而该替代物对用户交互过商品的语义相关性检索是不可靠，即检索到的商品，与LLM真正需要的长期兴趣存在很大的差距，生成式推荐的性能严重下降。


In the context of the LLM-based discriminative recommendation of judging user preferences for given candidate items, the "memorize then retrieve" framework has emerged as a promising solution for modeling long histories~\cite{rella}. This approach stores users' extensive historical interactions in memory and retrieves relevant portions when needed for LLM use. When recent interactions do not provide sufficient information, the LLM can refer to user feedback on similar items retrieved from the long history to generate predictions for the candidate items. This strategy effectively models long-term interests while minimizing the overhead of processing the entire history. Functionally speaking, the framework also appears well-suited for LLM-based generative recommendation, provided an appropriate memorization and retrieval mechanism is designed. 

For LLM-based generative recommendation, memorization can still be achieved by storing raw or encoded historical interaction data; however, the retrieval mechanism becomes significantly more challenging. 
As candidate items are no longer provided, the retrieval process must depend on other local input information, such as recent historical interactions, to extract useful historical data for the LLM. 
In this context, simple retrieval methods (e.g., semantic retrieval) often fall short of providing meaningful retrieval. For instance, when local input information is insufficient for generating accurate recommendations, semantic retrieval does not provide useful information to enhance the recommendations, as the retrieved results typically resemble the local data and fail to introduce new insights. Furthermore, it is difficult to heuristically identify which aspects of long-term interests are relevant in a specific scenario, complicating the manual design of effective retrieval strategies.

Given these considerations, we propose teaching the retriever to automatically learn how to extract useful information from memory, inspired by~\cite{Hamed_Zamani}. Specifically, we design an external memory-retriever module for LLMs, where the memory stores encoded historical interactions, and the retriever is a learnable network capable of identifying relevant elements from the memory and incorporating them into the LLM's input in a prefix manner to guide recommendations. To train the retriever for effective retrieval, we first manually insert each memory element into the LLM and evaluate its ability to reduce the perplexity (PPL) of target items, using this outcome as a relevance label. The labeled data is then used to train the retriever, enabling it to learn patterns for identifying effective elements from the memory automatically. Since the core of our method lies in leveraging the memory well with the automatic retrieval, we name it \textit{MemoRec}. 

The main contributions are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We highlight the importance of modeling long-term history for generative LLM-based recommendation and emphasize the potential of the memory-retrieval framework as a solution.
    
    % To the best of our knowledge, this is the first work to explore the integration of users' long-term interest in generative recommendation scenarios.
    
    % \item We propose a novel framework MemoRec for defining users' relevant long-term interests by equipping a pre-trained LLM-based generative recommendation model with an independent long-term interest retrieval model.
    \item  We propose MemoRec, a novel memory-retrieval framework that enables automatic learning of how to extract useful information from memory to support next-item generation within LLMs.
    
    \item We conduct extensive experiments on two widely used datasets, showing that MemoRec effectively improves the ability of LLMs to leverage long-term interests for generative recommendation.
\end{itemize}



% *******************************************************



% As a widely used technique in NLP, Retrieval-Augmented Generation (RAG) has been applied to recommendation systems powered by LLMs. Rella employs semantic similarity retrieval to search a memory bank composed of item titles interacted with by the user, using the target item’s title as a query. It then replaces the more temporally recent interacted items in the instruction with those that are semantically more relevant, determining whether the target item is worth recommending. However, there are two key limitations: (1) The concept of the target item exists only in discriminative recommendation scenarios; (2) In generative recommendation scenarios, where no explicit target item is available, the user's short-term interaction history must be used as a substitute for the target item in semantic retrieval. This substitution is unreliable, as the retrieved items often exhibit a significant gap from the long-term interests that the LLM truly requires. Consequently, the performance of the generative recommendation suffers considerable degradation.

% 我们认为，RAG在大语言模型生成式推荐场景下的应用包含如下两个核心挑战：一是关于检索：对于LLM生成下一个商品，如何定义哪些长期历史兴趣是相关的。检索能够识别哪些长期兴趣和短期兴趣结合后会增强生成能力，简单的检索如语义检索会造成长短期兴趣的冲突和大语言模型的不理解。二是检索模型应该做到快速低成本。例如常见的通过端到端的方式训练检索模型是不现实的，该方法会将所有历史注入LLM中，训练出筛选有效检索模型，然而，这种方式训练和推理的成本高昂且耗时严重。
% We identify two core challenges in applying RAG to generative recommendation scenarios with LLMs:

% 1. \textbf{Retrieval Challenge}: For LLMs tasked with generating the next item, how can we define which long-term interests are relevant? Retrieval should identify long-term interests that, when combined with short-term interests, enhance the generative capability of the LLM. Simple retrieval approaches, such as semantic retrieval, may lead to conflicts between long- and short-term interests and hinder the LLM's understanding.

% 2. \textbf{Efficiency and Low Cost}: Retrieval models should be fast and cost-effective. Training a retrieval model for LLM in an end-to-end manner is simply accessible but impractical. This approach involves injecting all historical data into the LLM and optimizing the retrieval model based on the LLM's loss. However, such a method is both computationally expensive and time-consuming during training and inference, making it unsuitable for efficient deployment.

% 为了达到这个目标，我们提出了MomeRec。MemoRec为一个已训练好的LLM生成式推荐模型（BIGRec），训练了一个独立的长期兴趣检索模型，以prefix的方式将检索到的最优长期兴趣加入该BIGRec中增强生成。首先将每条用户长期历史交互块（长期兴趣）的表示以prefix的方式插入到BIGRec中，获得BIGRec输出的ppl下降程度。其次，通过最小化检索分数的分布和ppl下降程度的分布来训练一个检索模型（MLP）。该方法定义的最相关的长期兴趣（ppl下降程度最大）有助于BIGRec在融合长短期兴趣后，命中用户当前最感兴趣的商品。更多的，我们观察到，MemoRec不仅对长期历史的检索结果的优劣具有很强的鲁棒性，即能够在长短期历史中择优输出，更能够达到1+1>2的效果。
% To address this challenge, we propose \textbf{MemoRec}. MemoRec enhances a pre-trained LLM-based generative recommendation model (BIGRec) by training an independent long-term interest retrieval model. The retrieved optimal long-term interests are incorporated into BIGRec in the form of prefixes to improve its generative capability. Specifically, each block of the user's long-term interaction (representing long-term interests) is inserted into BIGRec as a prefix, and the resulting decrease in perplexity (PPL) is used to evaluate its relevance. Then, a retrieval model (an MLP) is trained by minimizing the distribution gap between the retrieval scores distribution and the PPL reduction distribution. This approach ensures that the most relevant long-term interests (those causing the greatest PPL reduction) are retrieved, enabling BIGRec to better combine long- and short-term interests and predict the items the user is currently most interested in. In our experiments, Memorec demonstrated excellent capabilities in retrieving and leveraging long-term interests.
% Moreover, in generation stage, we observe that the LLM (BIGRec) not only exhibits strong robustness in retrieving long-term interests, that is, it effectively prioritizes the most relevant information from both long- and short-term histories, but also can achieve a synergistic "1 + 1 > 2" effect.

% 总的来说，我们的贡献有三个方面：1. 在我们的知识范围内，这是第一个在生成式推荐场景下，探究结合用户长期历史做推荐的工作。2.提出了一种定义用户相关的长期兴趣的方法，为已训练好的LLM生成式推荐模型配备一个独立的长期兴趣检索模型，3. 我们在两个广泛使用的数据集上进行了大量实验，MemoRec提升了大模型结合长期兴趣做生成式推荐能力。






==> main/backup/1_intro_1218.tex <==
\section{Introduction}
% 大语言模型已在推荐系统中得到广泛的应用。当前研究者们致力于利用大语言模型强大的生成能力做生成式推荐，即大语言模型基于由用户的历史交互构成的指令直接生成该用户接下来可能喜欢的商品文本表示，如商品标题。一般而言，用户接下来会喜欢的商品，通常由当下用户的短期兴趣，以及用户长期的兴趣共同决定。用户长期的交互历史中，包含有大量的用户长期兴趣。如何在大语言模型做生成式推荐的设定下，筛选出相关的长期兴趣以及有效融合筛选出的长期兴趣与短期兴趣的方法，是当前的热点话题。

Recently, significant efforts~\cite{LLMRecSurvey} have been made to leverage the remarkable abilities of Large Language Models (LLMs) for recommendation tasks. Given LLMs' generative nature, a popular generative recommendation paradigm has emerged~\cite{bigrec,d3,genrec,lc-rec} --- teaching LLMs 
to leverage inputted historical interactions to
directly generate the next recommended item, without requiring predefined candidate items. In this paradigm, the inputted historical interactions provide user interest information, playing a pivotal role in determining the personalized item generation.
Due to computational costs and limited context windows, existing methods typically incorporate only the user's most recent interactions, overlooking longer histories. However, these extended histories encapsulate the user's long-term interests, a crucial aspect of user interests, neglecting which would inevitably lead to suboptimal performance.
% Due to the cost and limited context windows, existing work typically only incorporates the user's most recent interactions, neglecting longer histories. However, the long history captures the user's long-term interests, which is also an important aspect of recommendation.. Failing to model such information would undoubtedly result in suboptimal performance.
%%This paradigm shows the power of achieving promising results and exhibits some specific characteristics than other paradigms, e.g., global ranking abilities. 

% Large language models (LLMs) have been widely applied in recommendation systems. Currently, researchers are focusing on leveraging the powerful generative capabilities of LLMs to enable generative recommendation. In this paradigm, LLMs directly generate text representations of items (e.g., item titles) that a user is likely to prefer, based on instructions constructed from the user's historical interactions. Due to disadvantages in terms of cost and performance, LLM-based generative models focus on leveraging short-term interactions to generate items, while neglecting the modeling of long-term interactions. Generally, the items a user may prefer next are jointly determined by the user's short-term interests and long-term interests. A user's long-term interaction history contains abundant information about their long-term interests. A key research challenge in the context of generative recommendation with LLMs is how to effectively identify relevant long-term interests and integrate these with short-term interests. This has become a prominent topic in the field.

% RAG作为NLP中广泛使用的技术已经被应用于大语言模型推荐系统上。Rella利用目标商品标题对由用户交互过的商品标题构成的记忆库进行语义相关性检索，将指令中原有的时间更近邻的已交互商品替换为语义相关性更强的已交互商品，判别目标商品是否值得被推荐。然而，1. 目标商品仅仅存在于判别式推荐场景中；2. 在生成式推荐场景下，我们只有通过用户的短期历史交互代替目标商品做语义检索，而该替代物对用户交互过商品的语义相关性检索是不可靠，即检索到的商品，与LLM真正需要的长期兴趣存在很大的差距，生成式推荐的性能严重下降。

\wcb{To this end, we explore the ``memorize-then-retrieve'' framework in generative recommendation. This idea naturally aligns with the Retrieval-Augmented Generation (RAG) paradigm, which effectively models long histories while minimizing the computational overhead of processing the entire history. In Natural Language Processing (NLP), RAG typically involves two steps: (1) storing users' extensive historical interactions in memory, and (2) retrieving relevant portions when needed for use by LLMs. This raises a critical research question: “How can we identify the most relevant information to enhance the LLM to generate the right item?” One possible solution is to directly use each item in the candidate pool to perform semantic retrieval. However, this approach is suboptimal because it incurs significant computational overhead when generating a recommendation list, as the LLM must process an extremely large number of candidates and their associated retrievals for making a single recommendation. }

\wcb{In addition, if the retrieval process depends only on the user query, such as instructions derived from recent historical interactions, simple retrieval methods (e.g., semantic retrieval) often fail to provide the meaningful information required by the LLM. For instance, when local input information is insufficient for generating accurate recommendations, semantic retrieval often fails to enhance the results, as the retrieved data tends to mirror the local input without providing new insights. Moreover, identifying which aspects of long-term interests are relevant in a specific scenario is challenging, making it difficult to manually design effective retrieval strategies.}

% In the context of the LLM-based discriminative recommendation of judging user preferences for given candidate items, the "memorize then retrieve" framework has emerged as a promising solution for modeling long histories~\cite{rella}. This approach stores users' extensive historical interactions in memory and retrieves relevant portions when needed for LLM use. When recent interactions do not provide sufficient information, the LLM can refer to user feedback on similar items retrieved from the long history to generate predictions for the candidate items. This strategy effectively models long-term interests while minimizing the overhead of processing the entire history. Functionally speaking, the framework also appears well-suited for LLM-based generative recommendation, provided an appropriate memorization and retrieval mechanism is designed. 

% For LLM-based generative recommendation, memorization can still be achieved by storing raw or encoded historical interaction data; however, the retrieval mechanism becomes significantly more challenging. 
% As candidate items are no longer provided, the retrieval process must depend on other local input information, such as recent historical interactions, to extract useful historical data for the LLM. 
% In this context, simple retrieval methods (e.g., semantic retrieval) often fall short of providing meaningful retrieval. For instance, when local input information is insufficient for generating accurate recommendations, semantic retrieval does not provide useful information to enhance the recommendations, as the retrieved results typically resemble the local data and fail to introduce new insights. Furthermore, it is difficult to heuristically identify which aspects of long-term interests are relevant in a specific scenario, complicating the manual design of effective retrieval strategies.

\wcb{Given these considerations, we propose a framework that trains an external retriever module for LLMs to automatically learn how to extract useful information from memory, inspired by~\cite{Hamed_Zamani}. Specifically, it is necessary to identify the relevant elements in memory to serve as labels for the retriever. Unlike the rich and purely semantic information in queries of retriever in NLP, user queries in recommendation systems contain both semantic information and behavioral features. This motivates us to directly use the LLM's feedback as labels for retriever training. We treat each long-term interest of the user in memory as a prefix of this user's local query and record the LLM's perplexity reduction. Consequently, the retriever, as a learnable network, is trained by minimizing the distribution gap between the retrieval scores and the perplexity (PPL) reduction distributions. Since the core of our method lies in effectively leveraging memory through automatic retrieval, we name it \textit{MemoRec}.}

% Given these considerations, we propose teaching the retriever to automatically learn how to extract useful information from memory, inspired by~\cite{Hamed_Zamani}. Specifically, we design an external memory-retriever module for LLMs, where the memory stores encoded historical interactions, and the retriever is a learnable network capable of identifying relevant elements from the memory and incorporating them into the LLM's input in a prefix manner to guide recommendations. To train the retriever for effective retrieval, we first manually insert each memory element into the LLM and evaluate its ability to reduce the perplexity (PPL) of target items, using this outcome as a relevance label. The labeled data is then used to train the retriever, enabling it to learn patterns for identifying effective elements from the memory automatically. Since the core of our method lies in leveraging the memory well with the automatic retrieval, we name it \textit{MemoRec}. 



The main contributions are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We highlight the importance of modeling long-term history for generative LLM-based recommendation and emphasize the potential of the memory-retrieval framework as a solution.
    
    % To the best of our knowledge, this is the first work to explore the integration of users' long-term interest in generative recommendation scenarios.
    
    % \item We propose a novel framework MemoRec for defining users' relevant long-term interests by equipping a pre-trained LLM-based generative recommendation model with an independent long-term interest retrieval model.
    \item  We propose MemoRec, a novel memory-retrieval framework that enables automatic learning of how to extract useful information from memory to support next-item generation within LLMs.
    
    \item We conduct extensive experiments on two widely used datasets, showing that MemoRec effectively improves the ability of LLMs to leverage long-term interests for generative recommendation.
\end{itemize}



% *******************************************************



% As a widely used technique in NLP, Retrieval-Augmented Generation (RAG) has been applied to recommendation systems powered by LLMs. Rella employs semantic similarity retrieval to search a memory bank composed of item titles interacted with by the user, using the target item’s title as a query. It then replaces the more temporally recent interacted items in the instruction with those that are semantically more relevant, determining whether the target item is worth recommending. However, there are two key limitations: (1) The concept of the target item exists only in discriminative recommendation scenarios; (2) In generative recommendation scenarios, where no explicit target item is available, the user's short-term interaction history must be used as a substitute for the target item in semantic retrieval. This substitution is unreliable, as the retrieved items often exhibit a significant gap from the long-term interests that the LLM truly requires. Consequently, the performance of the generative recommendation suffers considerable degradation.

% 我们认为，RAG在大语言模型生成式推荐场景下的应用包含如下两个核心挑战：一是关于检索：对于LLM生成下一个商品，如何定义哪些长期历史兴趣是相关的。检索能够识别哪些长期兴趣和短期兴趣结合后会增强生成能力，简单的检索如语义检索会造成长短期兴趣的冲突和大语言模型的不理解。二是检索模型应该做到快速低成本。例如常见的通过端到端的方式训练检索模型是不现实的，该方法会将所有历史注入LLM中，训练出筛选有效检索模型，然而，这种方式训练和推理的成本高昂且耗时严重。
% We identify two core challenges in applying RAG to generative recommendation scenarios with LLMs:

% 1. \textbf{Retrieval Challenge}: For LLMs tasked with generating the next item, how can we define which long-term interests are relevant? Retrieval should identify long-term interests that, when combined with short-term interests, enhance the generative capability of the LLM. Simple retrieval approaches, such as semantic retrieval, may lead to conflicts between long- and short-term interests and hinder the LLM's understanding.

% 2. \textbf{Efficiency and Low Cost}: Retrieval models should be fast and cost-effective. Training a retrieval model for LLM in an end-to-end manner is simply accessible but impractical. This approach involves injecting all historical data into the LLM and optimizing the retrieval model based on the LLM's loss. However, such a method is both computationally expensive and time-consuming during training and inference, making it unsuitable for efficient deployment.

% 为了达到这个目标，我们提出了MomeRec。MemoRec为一个已训练好的LLM生成式推荐模型（BIGRec），训练了一个独立的长期兴趣检索模型，以prefix的方式将检索到的最优长期兴趣加入该BIGRec中增强生成。首先将每条用户长期历史交互块（长期兴趣）的表示以prefix的方式插入到BIGRec中，获得BIGRec输出的ppl下降程度。其次，通过最小化检索分数的分布和ppl下降程度的分布来训练一个检索模型（MLP）。该方法定义的最相关的长期兴趣（ppl下降程度最大）有助于BIGRec在融合长短期兴趣后，命中用户当前最感兴趣的商品。更多的，我们观察到，MemoRec不仅对长期历史的检索结果的优劣具有很强的鲁棒性，即能够在长短期历史中择优输出，更能够达到1+1>2的效果。
% To address this challenge, we propose \textbf{MemoRec}. MemoRec enhances a pre-trained LLM-based generative recommendation model (BIGRec) by training an independent long-term interest retrieval model. The retrieved optimal long-term interests are incorporated into BIGRec in the form of prefixes to improve its generative capability. Specifically, each block of the user's long-term interaction (representing long-term interests) is inserted into BIGRec as a prefix, and the resulting decrease in perplexity (PPL) is used to evaluate its relevance. Then, a retrieval model (an MLP) is trained by minimizing the distribution gap between the retrieval scores distribution and the PPL reduction distribution. This approach ensures that the most relevant long-term interests (those causing the greatest PPL reduction) are retrieved, enabling BIGRec to better combine long- and short-term interests and predict the items the user is currently most interested in. In our experiments, Memorec demonstrated excellent capabilities in retrieving and leveraging long-term interests.
% Moreover, in generation stage, we observe that the LLM (BIGRec) not only exhibits strong robustness in retrieving long-term interests, that is, it effectively prioritizes the most relevant information from both long- and short-term histories, but also can achieve a synergistic "1 + 1 > 2" effect.

% 总的来说，我们的贡献有三个方面：1. 在我们的知识范围内，这是第一个在生成式推荐场景下，探究结合用户长期历史做推荐的工作。2.提出了一种定义用户相关的长期兴趣的方法，为已训练好的LLM生成式推荐模型配备一个独立的长期兴趣检索模型，3. 我们在两个广泛使用的数据集上进行了大量实验，MemoRec提升了大模型结合长期兴趣做生成式推荐能力。






==> main/backup/4_method.tex <==
\section{Preliminaries}
\label{Preliminaries}
Consider a recommender dataset $\mathcal{D} = \{(u, i_t, C_t^s, t)_n \ | \ n \in [1, N], t \in T\}$, where the user $u$ belongs to $U$, and the item $i_t \in I$ is the item the user intends to interact with at time step $t$, and $C_t^s$ represents the context consisting of the $m$ most recent items the user has interacted with up to step $t$. The total number of samples in the dataset is $N$. In the context of LLM-based generative recommendation, a large value of $m$ significantly increases the computational cost and inference latency. Therefore, $m$ is typically set to 10 during both training and inference. In this study, $C_t^s$ is referred to as the short-term context, representing the user's short-term interests.

For a given user, $\mathcal{D}_{u,t_k}^l = \{(u, i_t, C_t^s, t) \ | \ t < t_k\}$ contains all the user's historical interactions prior to step $t_k$, along with their corresponding $C_t^s$. In this paper, $C_{u,t_k}^l = \{C_t^s \ | \ C_t^s \in \mathcal{D}_{u,t_k}^l\}$ is defined as the long-term context set, which represents the user's long-term interests.

In LLM-based generative recommendation, the short-term context $C_t^s$ in the dataset is typically transformed into a textual instruction, such as: "This user has interacted with [Item title1], [Item title2], ..., [Item title n]. Please predict the next item the user is likely to engage with:", denoted as $x$, where [Item title] is derived from $C_t^s$. The LLM is then trained using an autoregressive objective function \ref{eq1}, where the response $y$ corresponds to the textual token sequence of the target item $i$, i.e., $y = y_1, y_2, ..., y_m$.
\begin{equation}\label{eq1}
    \max_\Phi\sum_{(x,y)\in\mathcal{D}}\sum_{i=1}^{|y|}\log(P_\Phi(y_i|x,y_{<i})),
\end{equation}
where the $\phi$ represents the parameters of the LLM, $y_i$ denotes the $t$-th token of $y$, and $y_{<i}$ represents the tokens preceding $y_i$.

During the recommendation phase, the LLM first generates tokens autoregressively based on the instruction constructed from $C_t^s$. The generated tokens are then mapped onto existing items in the dataset using a grounding mechanism, typically by minimizing the L2 distance between the generated tokens and representations of the items in the dataset.

\section{MemoRec}
To enable LLMs to effectively leverage users' long-term interests for recommendations in a generative recommendation setting, we propose MemoRec. In this section, we first define the methodology for integrating long-term and short-term interests. Based on this approach, we outline how to construct a relevant long-term interest dataset. Subsequently, using this dataset, we equip the LLM with an efficient and lightweight retrieval model designed to retrieve relevant long-term interests.

\subsection{Retrieval as prefix.}
For each user, we select the long-term interest that is most relevant to the current prediction task and prepend it as a prefix to the instruction constructed from the short-term interests. In contrast to approaches that replace or integrate interests through additional modules, this method offers a straightforward and efficient way to integrate long-term and short-term interests in chronological order, aligning well with the temporal evolution patterns captured by LLM during fine-tuning. Therefore, it has the potential to prevent a decline in the model's comprehension capabilities and eliminates the need for additional training of the LLM. Furthermore, the retrieval model constructed based on this approach is applicable to both black-box and white-box LLMs.

\subsection{Construct relevant samples.}
Based on the aforementioned prefix integration method, we define what constitutes relevant long-term interests. Relevant long-term interests can enhance the LLM's understanding of instructions and its ability to generate the target item. Therefore, for the sample $(u, i_{t_{k}}, C_{t_{k}}^{s}, t_{k})$ in the training set, we calculate the impact of each long-term interest in \( D_{u,t_k}^l = \{(u, i_t, C_t^{s}, t) \mid t < t_k\} \) on the output perplexity of the LLM (PPL) after adding it as a prefix to the instruction, as shown in Equation~\ref{eq2}:

\begin{equation}\label{eq2}
    \mathrm{ppl_{t_{k},t_{q}}^{u}}=\exp\left\{-\frac{1}{|y|}\sum_i^{|y|}\log p_\phi(y_i|y_{<i})\right\}
\end{equation}
\begin{equation}\label{eq3}
    \delta\mathrm{ppl_{t_{k},t_{q}}^u}= \mathrm{ppl_{t_{k},t_{q}}^u - ppl_{t_{k}}^u},
\end{equation}

where, $\text{t}_{\text{q}} < \text{t}_{\text{k}}$, $C_{t_{q}} \in C_{u,t_k}^l$ and $\text{ppl}_{t_{k}}^u$ denotes the ppl obtained by short-term interest only. A larger decrease in PPL indicates that the long-term interest contributes more to the LLM's generation of the target item, i.e., it is more relevant. Finally, based on Equation~\ref{eq3}, we obtain $ \Delta \text{PPL}_{t_k}^u = \{\delta \text{ppl}_{t_k,t_0}^u, \delta \text{ppl}_{t_k,t_1}^u, \ldots, \delta \text{ppl}_{t_k,t_{k-1}}^u\} $.

\subsection{Training of retriever.}
Our goal is to train a lightweight retrieval model capable of assigning higher retrieval scores to relevant long-term interests of user.

\subsubsection{Retrieval model architecture.}
We employ a simple Multi-Layer Perceptron (MLP) as the retrieval model. The query input for the retrieval model is the LLM embedding of instruction constructed from user's short-term interest $C_t^{s}$. Similarly, the retriever's key input is the LLM embedding of the user's long-term interests. The retrieval score distribution is computed using the following equation~\ref{eq4}:  
\begin{equation}\label{eq4}
\pi_\theta(C_{t_{q}}^s|C_{t_k}^s)=\frac{\exp\left(\mathcal{R}_\theta(l_\phi(C_{t_k}^s),l_\phi(C_{t_q}^s)\right)}{\sum_{C_{t_q^{\prime}}^s\in C_{u,t_k}^l}\exp\left(\mathcal{R}_\theta(l_\phi(C_{t_k}^s),l_\phi(C_{t_q^{\prime}}^s))\right)}:\forall C_{t_q}^s\in C_{u,t_k}^l,
\end{equation}
where $\mathcal{R}_\theta$ denotes the retrieval model parameterized by $\theta$, $l_{\phi}$ is the final embedding from the last layer of the LLM, and $C_{u,t_k}^l$ is the set of user's long-term interests prior to step $t_k$ (mentioned in Section~\ref{Preliminaries}).
\subsubsection{Optimizing Retriever.}

Based on \( \Delta \text{PPL}_{t_k}^u \), for the user’s sample $(u, i_{t_{k}}, C_{t_{k}}^{s}, t_{k})$ at step \( t_k \), we derive the golden probability distribution using the following equation~\ref{eq5}:  

\begin{equation}\label{eq5}
P_{g}(C_{t_{q}}^s|C_{t_k}^s)=\frac{\exp\left(\delta \text{ppl}_{t_k,t_q}^u\right)}{\sum_{t_q^{\prime} < t_k}\exp\left(\delta \text{ppl}_{t_k,t_{q^{\prime}}}^u\right)}:\forall \delta \text{ppl}_{t_k,t_q^{\prime}}^u \in \Delta \text{PPL}_{t_k}^u.
\end{equation}

We optimize the retrieval model by minimizing the KL divergence between the retrieval score distribution and the target probability distribution using the following equation~\ref{eq6}:  

\begin{equation}\label{eq6}
\arg\min_\theta\frac{1}{|B|}\sum_{(u,i_{t_{k}},C_{t_k}^s)\in B}\sum_{C_{t_q}^s\in D_{u,t_k}^l}P_{g}(C_{t_{q}}^s|C_{t_k}^s)\log\frac{\pi_\theta(C_{t_{q}}^s|C_{t_k}^s)}{P_{g}(C_{t_{q}}^s|C_{t_k}^s)},
\end{equation}
where $B$ denotes the mini-batch.

==> main/backup/5_experiment_backup_1211_chengbin.tex <==
\section{EXPERIMENTS}
In this section, we conduct experiments to answer the following research questions: \textbf{RQ1:} ?
\textbf{RQ2:}



\subsection{Experimental Setup}
% -------------------------1211 tianhao
\noindent \textbf{Datasets.} We conduct experiments on two representative datasets from Amazon Product Reviews\footnote{\url{https://jmcauley.ucsd.edu/data/amazon/}.}: Amazon Book (Book) and Amazon Movie (Movie). These datasets contain user reviews from Amazon, collected from 1996 to 2018, with scores ranging from 1 to 5. We transform these scores into binary using a threshold of 4. Due to the large scale of Amazon Review datasets, we extract data from 2017 for our experiments, allocating the first 10 months for training and long-term memory retrieval, and the remaining two halves for validation and testing, respectively. 
As this work studies long-term user interest, we filter out users with fewer than 20 interactions. 
To ensure data quality, we also filter out infrequent items with fewer than 5 interactions.
% To evaluate the sequential recommendation, we use the 放在details


\noindent \textbf{Baselines.} To evaluate the performance of text-rich sequential recommendations, we select several representative methods as baselines, including 1) SASRec~\cite{sasrec}, which is a traditional sequential recommendation method that uses a self-attention mechanism to grasp sequential patterns; 
2) BIGRec~\cite{bigrec}, which is an LLM-based generative recommendation model that grounds the output of LLM to actual item space using an L2 distance;
3) ReLLa~\cite{rella}, which models long-term user interest in discriminative recommendations by semantically retrieving the most relevant historical interactions to the target item. In generative recommendations, as the target item is unavailable, we adapt ReLLa by using the short-term item history as the query for retrieval; 4) TRSR~\cite{trsr}, 


\noindent \textbf{Evaluation metrics.} We adopt two widely used metrics to evaluate the top-K recommendation quality: Recall, and Normalized Discounted Cumulative
Gain (NDCG). 

\noindent \textbf{Implementation details.}

% We conduct experiments on two representative datasets: Amazon Book (Book) and Amazon Movie (Movie).





\subsubsection{Datasets}
%我们从两个广泛使用的真实数据集做实验 Amazon book and movies。这两个数据集都含有大量长期用户，有助于我们验证我们方法结合长短期兴趣的能力。我们抽取2017年的数据作为实验数据集，且将10月之前的数据作为训练集，11和12月的数据作为验证和测试。为了公平比较（不增加额外的数据），我们指定为训练集为能够获得的长期兴趣记忆库，即检索的对象仅限于在训练集中检索。在训练集中我们将交互次数少于5的不热门的用户和商品过滤掉，同时过滤掉验证和测试集中在记忆库中交互次数多于20次，少于100次的用户，保证我们测试的对象是长期用户。同时将过滤后的11和12月份数据按照时间顺序1:1划分为验证集和测试集。此外，按照我们保留最后 10 次交互作为历史序列用于训练生成式推荐模型，在本文中，该历史序列被称为短期上下文（兴趣）。
We conduct experiments using two widely adopted real-world datasets, Amazon Books (Book) and Amazon Movies (Movie). These datasets contain a significant number of long-term users, which allows us to evaluate the capability of our method to integrate long- and short-term interests effectively.  

We extracted data from 2017 for our experiments, using data prior to October as the training set, while data from November and December served as the validation and test sets. To ensure a fair comparison (without introducing additional data), we designated the training set as the only available long-term interest memory bank, meaning retrieval was restricted to items present in the training set.  

In the training set, we filtered out infrequent users and items with fewer than five interactions. Additionally, we excluded users in the validation and test sets who had more than 20 or fewer than 100 interactions in the memory bank to ensure that the evaluation focused on long-term users. The filtered data from November and December was then split 1:1 in chronological order into the validation and test sets.  

Following standard practices, we retained the last 10 interactions as the historical sequence for training and testing the generative recommendation models (baselines). In this work, this historical sequence is referred to as the short-term context (interest).



\subsubsection{backbone and Baselines}
%我们选择了一个最常见的传统模型SASRec以及两个最新的专注于LLM场景下建模长期用户兴趣的方法：1）R e L L a：在LLM判别式推荐场景下，ReLLa通过目标商品的语义信息，对用户的历史交互商品进行召回，通过将由时间近邻的构造的指令替换为语义近邻来判断目标商品是否值得被推荐。然而在生成式推荐场景下，目标商品是无法获得的，故而我们在本文中，通过短期交互历史作为替代做语义检索。2）TRSR：该方法通过LLM的总结能力，对用户的所有交互历史生成总结文本，然后将用户的总结和用户的短期兴趣构建为指令，微调LLM。
We select state-of-the-art LLM-based generative recommendation model BigRec as our backbone. BigRec performs recommendation in two stages: First, it generates tokens based on instructions constructed from the user's short-term context. Then, it maps the LLM embeddings of these tokens to existing items in the dataset using L2 distance.

In addition to BigRec, we also selected three baselines including one of the most common traditional models, SASRec~\cite{sasrec}, and two state-of-the-art methods focused on modeling long-term user interests in LLM-based recommendation scenarios: 1) ReLLa~\cite{rella}: In the discriminative recommendation setting with LLMs, ReLLa retrieves the user’s interaction items in memory based on the semantic information of the target item. It replaces time-based neighbors in instructions with semantically similar neighbors to determine whether the target item is worth recommending. However, in the generative recommendation setting, the target item is not available. Therefore, in this work, we adapt ReLLa by using short-term interaction history as a substitute for semantic retrieval. 2) TRSR~\cite{trsr}: This method leverages the summarization capabilities of LLMs to generate a summary of the user’s preferences of all interaction items in memory. It then combines the user's summary with their short-term context to construct an instruction for fine-tuning the LLM.  


\subsubsection{Metrics}
We use two commonly used metrics, Recall and NDCG as the evaluation metrics.
To evaluate the model’s top-K recommendation performance, we use two commonly used
metrics: Recall@K and NDCG@K, which we compute in the all-ranking evaluation setting. In this paper, we set K as 1 and 5. 
\subsubsection{Implementation details}
For the SASRec, we conduct a grid search for learning rate and weight decay searched in [1e-2, 1e-3, 1e-4] and batch size within the range of [256,512,1024,2048]. The model is optimized by using BCE loss and the Adam optimizer. For LLM-based methods (BigRec, \zjz{ReLLa}, TRSR), we apply Llama2-7B as the LLM backbone. we use the AdamW optimizer and adjust the learning rate within the range of [1e-3, 1e-4, 5e-5]. During the training, we adjust the learning rate over steps using a cosine scheduler and set the early stop strategy based on Recall@1 metric. For training retriever, we adopted the same experimental setting with SASRec including search range of the learning rate, weight decay, batch size and the Adam optimizer. We also search the temperature coefficient in KL-loss within the range of [10, 1, 0.1, 0.01]. All experiments were conducted on an \zjz{NVIDIA A100 GPU}.

% \subsection{Comparison with State-of-the-arts}
\subsection{Results}



\begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.4}
\caption{The comparison between MemoRec and baselines.}
\label{table2} 
\begin{tabular}{lcccc}
\toprule
Dataset                & Model   & Recall@1 & Recall@5 & NDCG@5 \\
\hline
\multirow{5}{*}{Book}  & SASRec  & 0.0047   & 0.0214   & 0.0128 \\
                       & ReLLa   & 0.0045   & 0.0065   & 0.0055 \\
                       & TRSR    & \underline{0.0283}   & 0.0351   & 0.0319 \\
                       & BigRec  & 0.0281   & \underline{0.0360}   & \underline{0.0323} \\ \cline{2-5}
\rowcolor[HTML]{E9E9E9}                       & MemoRec & \textbf{0.0291}   & \textbf{0.0379}   & \textbf{0.0338} \\
\hline
\multirow{5}{*}{Movie} & SASRec  & 0.0329   & 0.0554   & 0.0437 \\
                       & ReLLa   & 0.0029   & 0.0050   & 0.0030  \\
                       & TRSR    & \underline{0.0591}   & \underline{0.0637}   & \underline{0.0613} \\
                       & BigRec  & 0.0575   & 0.0616   & 0.0597 \\ \cline{2-5}
\rowcolor[HTML]{E9E9E9}                       & MemoRec & \textbf{0.0601}   & \textbf{0.0638}   & \textbf{0.0621} \\
\bottomrule
\end{tabular}
\end{table}

% 在这个章节里，我们比较了提出的MemoRec和baselines的整体性能。正如表2中展示的，MemoRec在两个数据集的测评指标Recall@1， Recall@5 ，NDCG@5上超越了所有的baselines。该方法为BigRec配备的长期兴趣检索模型，引入了长期兴趣，在BigRec的基础上得到了明显的增益。更多地，比较当前存在的基于LLM的利用长期兴趣的方法（ReLLa，TRSR），我们的方法是一种更高效的方式。值得注意的是，ReLLa在所有数据和指标上，均表现出较差的推荐性能，这是因为ReLLa是在判别式推荐场景下提出的，而在生成式推荐场景下，仅仅能够使用短期兴趣的语义表示代替目标商品对长期兴趣检索，严重限制了ReLLa的性能。TRSR在两个数据集上表现出了不稳定的性能，在Book数据集上，以长期兴趣的总结与短期兴趣融合导致了性能的损失（对比BigRec），这是由于长期兴趣的总结会丢失大量的用长期兴趣，而且十分依赖LLM的总结能力。综上所述，我们提出的方法，在基于LLM的生成式推荐场景下，能够检索到LLM真正需要的长期兴趣，故而展现出了高效且稳定的融合长短期兴趣做推荐的能力。
\subsection{Overall performance comparison.}

In this section, we compare the overall performance of the proposed MemoRec with baselines. As shown in Table~\ref{table2}, MemoRec outperforms all baselines across both datasets in terms of the evaluation metrics Recall@1, Recall@5, and NDCG@5. 

MemoRec integrates a long-term interest retrieval model into BigRec, resulting in significant improvements over the original BigRec. Furthermore, when compared to existing LLM-based methods that utilize long-term interests such as ReLLa and TRSR, our method demonstrates a more effective approach. 

$\bullet$  ReLLa exhibits the poorest recommendation performance across all datasets and metrics. This is because ReLLa was designed for discriminative recommendation scenarios, and in generative recommendation scenarios, it can only use the semantic representation of  local input information instead of target item to retrieve long-term interests, which severely limits its performance. 

$\bullet$  TRSR shows unstable performance across the two datasets. Specifically, on the Book dataset, the integration of long-term historical summaries with local input information leads to a performance loss (compared to BigRec). This is due to the fact that summarizing a user's entire history into a single summarized text results in the loss of a large amount of long-term interests and heavily relies on the summarization capabilities of the LLM. 

In conclusion, our proposed method can retrieve the long-term interests genuinely needed by the LLM in generative recommendation scenarios, thereby demonstrating an efficient and stable ability to recommend by integrating both long-term and short-term interests.

\subsection{Analysis}
\begin{figure}[tbp]
  \centering            
  \subfloat[]{
        \label{fig:book_wrand}\includegraphics[width=0.25\textwidth]{Fig/book_wrand.pdf}}
   \subfloat[]{
        \label{fig:movie_wrand}\includegraphics[width=0.25\textwidth]{Fig/movie_wrand.pdf}} 
  % \caption{The timestamps of user's next interaction for augmentable and non-augmentable users.}
  \caption{The comparison between MemoRec and random retrieval.}
  \label{fig:wrand}
\end{figure}

\begin{figure}[tbp]
  \centering            
  \subfloat[]{
        \label{fig:bm_timestamp}\includegraphics[width=0.22\textwidth]{Fig/bm_timestamp.pdf}}
  \subfloat[]{
        \label{fig:case_study}\includegraphics[width=0.27\textwidth]{Fig/case_study.pdf}}
  \caption{(a) The timestamps of user's interaction at test time for augmentable and non-augmentable users. "True" means the MemoRec can enhance the recommendation for this interaction of the user.  (b) Case study: the interaction times of the user's relevant long-term interests which is obtained by MemoRec.}
  \label{fig:DNS}
\end{figure}


% 消融实验
% 
\subsubsection{Ablation study of retriever.}
% 为了验证我们检索器的有效性，我们展示了我们训练得到的检索器和随机检索的性能比较。如图1，MemoRec在两个数据集均比随机检索高且性能的提升具有鲁棒性。具体地，MemoRec在所有指标上的中位数均比随机检索高。不仅如此，其25 百分位数均高于随机检索的中位数，这是由于MemoRec相对于随机检索能够有效避免检索到有害的内容。
% To evaluate the effectiveness of our retriever, we present a performance comparison between our MemoRec and random retrieval. As shown in Figure 1, MemoRec consistently outperforms random retrieval across both datasets, demonstrating robust performance improvements. Specifically, the median performance of MemoRec on all metrics is higher than that of random retrieval. Furthermore, the 25th percentile of MemoRec's performance surpasses the median of random retrieval. This is attributed to MemoRec's ability to effectively avoid retrieving harmful content compared to random retrieval.

To validate the effectiveness of MemoRec, we present a performance comparison with random retrieval. As shown in Figure~\ref{fig:wrand}, MemoRec outperforms random retrieval across both datasets, and its retrieval performance demonstrates robustness. Specifically, the median performance of MemoRec on all metrics, as well as its 25th percentile, is higher than the median of random retrieval. This improvement is attributed to MemoRec's ability to effectively avoid retrieving harmful long-term interest compared to random retrieval.

\subsubsection{Key factor of retireval.}
% 我们发现MemoRec能否增强推荐与用户的交互时间这一关键因素有关。MemoRec有潜力根据在数据集上用户表现出来的与交互时间相关的潜在行为模式进行检索，并增强推荐。如图1，根据能否被MemoRec检索增强分为的2组用户交互之间存在很明显的交互时间差异。在movie数据集上，MemoRec能为与历史时间相距不太远的交互行为进行检索增强推荐，这可能是因为该数据集包含一个潜在的用户行为模式，即用户一般在短期内会被刚看完的一场电影所影响，。而在book数据集的书籍更倾向于对用户兴趣的长期影响，故而MemoRec能增强与历史交互时间相距较远的交互。同时，该现象能够进一步加强table1中的结论，即不像trsr，MemoRec能够根据不同数据集中用户的潜在行为模式提供稳定的增强效果。
% Figure~\ref{fig:bm_timestamp} illustrates that whether MemoRec can enhance recommendations is closely related to the time of user interaction, and the time of interactions which can be enhanced focused on a . As Figure~\ref{fig:bm_timestamp} shows, there is a significant difference in interaction time between the two groups of users, categorized based on whether their interactions can be enhanced by MemoRec. 

% In the Movie dataset, MemoRec is capable of enhancing recommendations for interactions that occurred relatively close in time to interactions in memory. This may be due to the fact that the movie dataset involves an underlying pattern of user behavior, i.e., users are generally influenced by recently watched movies over a short period. In contrast, in the Book dataset, books may tend to have a more long-term influence on user interests. As a result, MemoRec is able to enhance interactions that are further removed from interaction times in memory.

% 图~ref{fig:bm_timestamp}说明，MemoRec 能否增强推荐效果与用户交互的时间密切相关，且能被增强的用户交互主要发生在特定的时间范围内，我们将其称作增强时间区间。增强时间区间存在并且会随着数据集变化，一个可能的原因是由于数据集中商品的特点，用户受到长期兴趣的影响的时间范围不同，而memorec能够有效的捕捉到该时间范围做增强推荐。
% 增强时间间隔存在并且会随着数据集变化，一个可能的原因是由于数据集中的项目的特性和差异性，这会导致该数据平台上用户在特定的时间范围内会显著地受到长期兴趣的影响。
Figure~\ref{fig:bm_timestamp} demonstrates that the effectiveness of MemoRec in enhancing recommendations is closely associated with the timing of user interactions. Specifically, user interactions that can be enhanced predominantly occur within a specific time range, which we refer to as the enhancement time interval. 
The presence of the enhancement time interval, as well as its variation across datasets, may be attributed to the characteristics of the items within the datasets, which may lead to users on this data platform being significantly influenced by long-term interests within a specific time range.
MemoRec is capable of effectively capturing this time range to perform enhanced recommendations.

This observation further reinforces the conclusion in Table~\ref{table2}: unlike TRSR, MemoRec provides stable augmentation effects by capturing enhancement time intervals across different datasets.

\subsubsection{Case study.}
% 我们通过图1展示了用户被检索的相关长期兴趣的交互时间。图中，MemoRec能够成功检索时间上很久远的用户长期兴趣，这也为用户终身推荐系统的构建提供了可能。
Figure~\ref{fig:case_study} is a case study showing the interaction times of user's relevant long-term interests retrieved by MemoRec.
This figure shows that MemoRec successfully retrieves users' long-term interests even from distant past interactions, which opens up possibilities for building lifelong generative recommendation powered by LLM.










































% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/case_study.pdf}
%   \caption{% 用户的长期兴趣以及MemoRec检索到的该用户相关长期兴趣的出现时间。
%   Case study: The timestamps of user's long-term interests and the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}





% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/movie_posi_his_time_user.pdf}
%   \caption{
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}


% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/bm_time_rand.pdf}
%   \caption{
%   The timestamps of the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}



% \begin{figure*}[tbp]
%   \centering            
%   \subfloat[local-time]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.33\textwidth]{Fig/compare_wrand.pdf}}
%   \subfloat[local-time-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.33\textwidth]{Fig/bm_local_time.pdf}}
%   \subfloat[local-time-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.33\textwidth]{Fig/case_study.pdf}}
%   \caption{The timestamps of user's next interaction for augmentable and non-augmentable users.}
%   \label{fig:DNS}
% \end{figure*}

% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/compare_wrand.pdf}
%   \caption{
%   The retrieval capability of MemoRec compared to random retrieval.
%   }
%   \label{}
% \end{figure}




% \begin{table}[]
% % \centering
% \caption{The statistics of datasets.}
% \begin{tabular}{ccccc}
% \hline
% Dataset &$\#$Users    &$\#$Items    &train  &test   \\
% \midrule
% Book      &15,400 &1,000 &311,704 &48,600 \\
% Movie     &1411 &3327 &1,934,404 &2,742,166 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[tbp]
%   \centering            
%   \subfloat[his-len]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.25\textwidth]{Fig/bm_his_len.pdf}}
%   \subfloat[his-len-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.25\textwidth]{Fig/bm_his_len_rand.pdf}}
%   \caption{% 能够被增强的用户和不能被增强的用户的历史兴趣长度
%   Historical length of interest for users who can be augmented and users who cannot be augmented.
%   }
%   \label{fig:DNS}
% \end{figure}

% \begin{figure}[tbp]
%   \centering            
%   \subfloat[local-rank-len]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.25\textwidth]{Fig/bm_local_rank.pdf}}
%   \subfloat[local-rank-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.25\textwidth]{Fig/bm_local_rank_rand.pdf}}
%   \caption{
%   The recommendation capabilities of short-term contexts for augmentable and non-augmentable users.
%   }
%   \label{fig:DNS}
% \end{figure}

% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/book_posi_his_time_user.pdf}
%   \caption{% 用户的长期兴趣以及MemoRec检索到的该用户相关长期兴趣的出现时间。
%   Case study: The timestamps of user's long-term interests and the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}




==> main/backup/expr.tex <==
\section{EXPERIMENTS}
\subsection{Experimental Setup}

\subsubsection{Datasets}
%我们从两个广泛使用的真实数据集做实验 Amazon book and movies。这两个数据集都含有大量长期用户，有助于我们验证我们方法结合长短期兴趣的能力。我们抽取2017年的数据作为实验数据集，且将10月之前的数据作为训练集，11和12月的数据作为验证和测试。为了公平比较（不增加额外的数据），我们指定为训练集为能够获得的长期兴趣记忆库，即检索的对象仅限于在训练集中检索。在训练集中我们将交互次数少于5的不热门的用户和商品过滤掉，同时过滤掉验证和测试集中在记忆库中交互次数多于20次，少于100次的用户，保证我们测试的对象是长期用户。同时将过滤后的11和12月份数据按照时间顺序1:1划分为验证集和测试集。此外，按照我们保留最后 10 次交互作为历史序列用于训练生成式推荐模型，在本文中，该历史序列被称为短期上下文（兴趣）。
We conducted experiments using two widely adopted real-world datasets, Amazon Books and Amazon Movies. These datasets contain a significant number of long-term users, which allows us to evaluate the capability of our method to integrate long- and short-term interests effectively.  

We extracted data from 2017 for our experiments, using data prior to October as the training set, while data from November and December served as the validation and test sets. To ensure a fair comparison (without introducing additional data), we designated the training set as the only available long-term interest memory bank, meaning retrieval was restricted to items present in the training set.  

In the training set, we filtered out infrequent users and items with fewer than five interactions. Additionally, we excluded users in the validation and test sets who had more than 20 or fewer than 100 interactions in the memory bank to ensure that the evaluation focused on long-term users. The filtered data from November and December was then split 1:1 in chronological order into the validation and test sets.  

Following standard practices, we retained the last 10 interactions as the historical sequence for training and testing the generative recommendation models (baselines). In this work, this historical sequence is referred to as the short-term context (interest).



\subsubsection{backbone and Baselines}
%我们选择了一个最常见的传统模型SASRec以及两个最新的专注于LLM场景下建模长期用户兴趣的方法：1）R e L L a：在LLM判别式推荐场景下，ReLLa通过目标商品的语义信息，对用户的历史交互商品进行召回，通过将由时间近邻的构造的指令替换为语义近邻来判断目标商品是否值得被推荐。然而在生成式推荐场景下，目标商品是无法获得的，故而我们在本文中，通过短期交互历史作为替代做语义检索。2）TRSR：该方法通过LLM的总结能力，对用户的所有交互历史生成总结文本，然后将用户的总结和用户的短期兴趣构建为指令，微调LLM。
We select state-of-the-art LLM-based generative recommendation model BigRec as our backbone. BigRec performs recommendation in two stages: First, it generates tokens based on instructions constructed from the user's short-term context. Then, it maps the LLM embeddings of these tokens to existing items in the dataset using L2 distance.

In addition to BigRec, we also selected three baselines including one of the most common traditional models, SASRec~\cite{sasrec}, and two state-of-the-art methods focused on modeling long-term user interests in LLM-based recommendation scenarios: 1) ReLLa~\citerella}: In the discriminative recommendation setting with LLMs, ReLLa retrieves the user’s interaction items in memory based on the semantic information of the target item. It replaces time-based neighbors in instructions with semantically similar neighbors to determine whether the target item is worth recommending. However, in the generative recommendation setting, the target item is not available. Therefore, in this work, we adapt ReLLa by using short-term interaction history as a substitute for semantic retrieval. 2) TRSR~\cite{trsr}: This method leverages the summarization capabilities of LLMs to generate a summary of the user’s preferences of all interaction items in memory. It then combines the user's summary with their short-term context to construct an instruction for fine-tuning the LLM.  


\subsubsection{Metrics}
We use two commonly used metrics, Recall and NDCG as the evaluation metrics.
To evaluate the model’s top-K recommendation performance, we use two commonly used
metrics: Recall@K and NDCG@K, which we compute in the all-ranking evaluation setting. In this paper, we set K as 1 and 5. 
\subsubsection{Implementation details}
For the SASRec, we conduct a grid search for learning rate and weight decay searched in [1e-2, 1e-3, 1e-4] and batch size within the range of [256,512,1024,2048]. The model is optimized by using BCE loss and the Adam optimizer. For LLM-based methods (BigRec, R e L L, TRSR), we apply Llama2-7B as the LLM backbone. we use the AdamW optimizer and adjust the learning rate within the range of [1e-3, 1e-4, 5e-5]. During the training, we adjust the learning rate over steps using a cosine scheduler and set the early stop strategy based on Recall@1 metric. For training retriever, we adopted the same experimental setting with SASRec including search range of the learning rate, weight decay, batch size and the Adam optimizer. We also search the temperature coefficient in KL-loss within the range of [10, 1, 0.1, 0.01]. All experiments were conducted on an A100 NVIDIA RTX GPUs.

% \subsection{Comparison with State-of-the-arts}
\subsection{Results}



\begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.4}
\caption{The comparison between MemoRec and baselines.}
\label{table2} 
\begin{tabular}{lcccc}
\toprule
Dataset                & Model   & Recall@1 & Recall@5 & NDCG@5 \\
\hline
\multirow{5}{*}{Book}  & SASRec  & 0.0047   & 0.0214   & 0.0128 \\
                       & ReLLa   & 0.0045   & 0.0065   & 0.0055 \\
                       & TRSR    & \underline{0.0283}   & 0.0351   & 0.0319 \\
                       & BigRec  & 0.0281   & \underline{0.0360}   & \underline{0.0323} \\ \cline{2-5}
                       & MemoRec & \textbf{0.0291}   & \textbf{0.0379}   & \textbf{0.0338} \\
\hline
\multirow{5}{*}{Movie} & SASRec  & 0.0329   & 0.0554   & 0.0437 \\
                       & ReLLa   & 0.0029   & 0.0050   & 0.0030  \\
                       & TRSR    & \underline{0.0591}   & \underline{0.0637}   & \underline{0.0613} \\
                       & BigRec  & 0.0575   & 0.0616   & 0.0597 \\ \cline{2-5}
                       & MemoRec & \textbf{0.0601}   & \textbf{0.0638}   & \textbf{0.0621} \\
\bottomrule
\end{tabular}
\end{table}

% 在这个章节里，我们比较了提出的MemoRec和baselines的整体性能。正如表2中展示的，MemoRec在两个数据集的测评指标Recall@1， Recall@5 ，NDCG@5上超越了所有的baselines。该方法为BigRec配备的长期兴趣检索模型，引入了长期兴趣，在BigRec的基础上得到了明显的增益。更多地，比较当前存在的基于LLM的利用长期兴趣的方法（ReLLa，TRSR），我们的方法是一种更高效的方式。值得注意的是，ReLLa在所有数据和指标上，均表现出较差的推荐性能，这是因为ReLLa是在判别式推荐场景下提出的，而在生成式推荐场景下，仅仅能够使用短期兴趣的语义表示代替目标商品对长期兴趣检索，严重限制了ReLLa的性能。TRSR在两个数据集上表现出了不稳定的性能，在Book数据集上，以长期兴趣的总结与短期兴趣融合导致了性能的损失（对比BigRec），这是由于长期兴趣的总结会丢失大量的用长期兴趣，而且十分依赖LLM的总结能力。综上所述，我们提出的方法，在基于LLM的生成式推荐场景下，能够检索到LLM真正需要的长期兴趣，故而展现出了高效且稳定的融合长短期兴趣做推荐的能力。
\subsection{Overall performance comparison.}

In this section, we compare the overall performance of the proposed MemoRec with baselines. As shown in Table~\ref{table2}, MemoRec outperforms all baselines across both datasets in terms of the evaluation metrics Recall@1, Recall@5, and NDCG@5. 

MemoRec integrates a long-term interest retrieval model into BigRec, resulting in significant improvements over the original BigRec. Furthermore, when compared to existing LLM-based methods that utilize long-term interests such as ReLLa and TRSR, our method demonstrates a more effective approach. 

$\bullet$  ReLLa exhibits the poorest recommendation performance across all datasets and metrics. This is because ReLLa was designed for discriminative recommendation scenarios, and in generative recommendation scenarios, it can only use the semantic representation of  local input information instead of target item to retrieve long-term interests, which severely limits its performance. 

$\bullet$  TRSR shows unstable performance across the two datasets. Specifically, on the Book dataset, the integration of long-term historical summaries with local input information leads to a performance loss (compared to BigRec). This is due to the fact that summarizing a user's entire history into a single summarized text results in the loss of a large amount of long-term interests and heavily relies on the summarization capabilities of the LLM. 

In conclusion, our proposed method can retrieve the long-term interests genuinely needed by the LLM in generative recommendation scenarios, thereby demonstrating an efficient and stable ability to recommend by integrating both long-term and short-term interests.

\subsection{Analysis}
\begin{figure}[tbp]
  \centering            
  \subfloat[]{
        \label{fig:book_wrand}\includegraphics[width=0.25\textwidth]{Fig/book_wrand.pdf}}
   \subfloat[]{
        \label{fig:movie_wrand}\includegraphics[width=0.25\textwidth]{Fig/movie_wrand.pdf}} 
  % \caption{The timestamps of user's next interaction for augmentable and non-augmentable users.}
  \caption{The comparison between MemoRec and random retrieval.}
  \label{fig:wrand}
\end{figure}

\begin{figure}[tbp]
  \centering            
  \subfloat[]{
        \label{fig:bm_timestamp}\includegraphics[width=0.22\textwidth]{Fig/bm_timestamp.pdf}}
  \subfloat[]{
        \label{fig:case_study}\includegraphics[width=0.27\textwidth]{Fig/case_study.pdf}}
  \caption{(a) The timestamps of user's interaction at test time for augmentable and non-augmentable users. "True" means the MemoRec can enhance the recommendation for this interaction of the user.  (b) Case study: the interaction times of the user's relevant long-term interests which is obtained by MemoRec.}
  \label{fig:DNS}
\end{figure}


% 消融实验
% 
\subsubsection{Ablation study of retriever.}
% 为了验证我们检索器的有效性，我们展示了我们训练得到的检索器和随机检索的性能比较。如图1，MemoRec在两个数据集均比随机检索高且性能的提升具有鲁棒性。具体地，MemoRec在所有指标上的中位数均比随机检索高。不仅如此，其25 百分位数均高于随机检索的中位数，这是由于MemoRec相对于随机检索能够有效避免检索到有害的内容。
% To evaluate the effectiveness of our retriever, we present a performance comparison between our MemoRec and random retrieval. As shown in Figure 1, MemoRec consistently outperforms random retrieval across both datasets, demonstrating robust performance improvements. Specifically, the median performance of MemoRec on all metrics is higher than that of random retrieval. Furthermore, the 25th percentile of MemoRec's performance surpasses the median of random retrieval. This is attributed to MemoRec's ability to effectively avoid retrieving harmful content compared to random retrieval.

To validate the effectiveness of MemoRec, we present a performance comparison with random retrieval. As shown in Figure~\ref{fig:wrand}, MemoRec outperforms random retrieval across both datasets, and its retrieval performance demonstrates robustness. Specifically, the median performance of MemoRec on all metrics, as well as its 25th percentile, is higher than the median of random retrieval. This improvement is attributed to MemoRec's ability to effectively avoid retrieving harmful long-term interest compared to random retrieval.

\subsubsection{Key factor of retireval.}
% 我们发现MemoRec能否增强推荐与用户的交互时间这一关键因素有关。MemoRec有潜力根据在数据集上用户表现出来的与交互时间相关的潜在行为模式进行检索，并增强推荐。如图1，根据能否被MemoRec检索增强分为的2组用户交互之间存在很明显的交互时间差异。在movie数据集上，MemoRec能为与历史时间相距不太远的交互行为进行检索增强推荐，这可能是因为该数据集包含一个潜在的用户行为模式，即用户一般在短期内会被刚看完的一场电影所影响，。而在book数据集的书籍更倾向于对用户兴趣的长期影响，故而MemoRec能增强与历史交互时间相距较远的交互。同时，该现象能够进一步加强table1中的结论，即不像trsr，MemoRec能够根据不同数据集中用户的潜在行为模式提供稳定的增强效果。
This section illustrates that whether MemoRec can enhance recommendations is closely related to the time of user interaction. As Figure~\ref{fig:bm_timestamp} shows, there is a significant difference in interaction time between the two groups of users, categorized based on whether their interactions can be enhanced by MemoRec. We claim that the interaction time involves users' behavioral patterns 
Figure~\ref{fig:bm_timestamp} illustrates that whether MemoRec can enhance recommendations is closely related to the time of user interaction. We observe that MemoRec has the potential to enhance recommendations based on users' behavioral patterns associated with interaction time. As shown in Figure~\ref{fig:bm_timestamp}, there is a significant difference in interaction time between the two groups of users, categorized based on whether their interactions can be enhanced by MemoRec.

In the Movie dataset, MemoRec is capable of enhancing recommendations for interactions that occurred relatively close in time to interactions in memory. 
This may be due to the fact that the movie dataset involves an underlying pattern of user behavior, i.e., users are generally influenced by recently watched movies over a short period. In contrast, in the Book dataset, books may tend to have a more long-term influence on user interests. As a result, MemoRec is able to enhance interactions that are further removed from interaction times in memory.

This observation further reinforces the conclusion in Table~\ref{table2}: unlike TRSR, MemoRec provides stable augmentation effects by adapting to different time-related behavioral patterns across different datasets.

\subsubsection{Case study.}
% 我们通过图1展示了用户被检索的相关长期兴趣的交互时间。图中，MemoRec能够成功检索时间上很久远的用户长期兴趣，这也为用户终身推荐系统的构建提供了可能。
Figure~\ref{fig:case_study} is a case study showing the interaction times of user's relevant long-term interests retrieved by MemoRec.
This figure shows that MemoRec successfully retrieves users' long-term interests even from distant past interactions, which opens up possibilities for building lifelong generative recommendation powered by LLM.










































% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/case_study.pdf}
%   \caption{% 用户的长期兴趣以及MemoRec检索到的该用户相关长期兴趣的出现时间。
%   Case study: The timestamps of user's long-term interests and the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}





% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/movie_posi_his_time_user.pdf}
%   \caption{
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}


% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/bm_time_rand.pdf}
%   \caption{
%   The timestamps of the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}



% \begin{figure*}[tbp]
%   \centering            
%   \subfloat[local-time]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.33\textwidth]{Fig/compare_wrand.pdf}}
%   \subfloat[local-time-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.33\textwidth]{Fig/bm_local_time.pdf}}
%   \subfloat[local-time-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.33\textwidth]{Fig/case_study.pdf}}
%   \caption{The timestamps of user's next interaction for augmentable and non-augmentable users.}
%   \label{fig:DNS}
% \end{figure*}

% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/compare_wrand.pdf}
%   \caption{
%   The retrieval capability of MemoRec compared to random retrieval.
%   }
%   \label{}
% \end{figure}




% \begin{table}[]
% % \centering
% \caption{The statistics of datasets.}
% \begin{tabular}{ccccc}
% \hline
% Dataset &$\#$Users    &$\#$Items    &train  &test   \\
% \midrule
% Book      &15,400 &1,000 &311,704 &48,600 \\
% Movie     &1411 &3327 &1,934,404 &2,742,166 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[tbp]
%   \centering            
%   \subfloat[his-len]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.25\textwidth]{Fig/bm_his_len.pdf}}
%   \subfloat[his-len-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.25\textwidth]{Fig/bm_his_len_rand.pdf}}
%   \caption{% 能够被增强的用户和不能被增强的用户的历史兴趣长度
%   Historical length of interest for users who can be augmented and users who cannot be augmented.
%   }
%   \label{fig:DNS}
% \end{figure}

% \begin{figure}[tbp]
%   \centering            
%   \subfloat[local-rank-len]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.25\textwidth]{Fig/bm_local_rank.pdf}}
%   \subfloat[local-rank-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.25\textwidth]{Fig/bm_local_rank_rand.pdf}}
%   \caption{
%   The recommendation capabilities of short-term contexts for augmentable and non-augmentable users.
%   }
%   \label{fig:DNS}
% \end{figure}

% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/book_posi_his_time_user.pdf}
%   \caption{% 用户的长期兴趣以及MemoRec检索到的该用户相关长期兴趣的出现时间。
%   Case study: The timestamps of user's long-term interests and the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}




==> main/backup/expr1219.tex <==
\section{\zjz{Experiments}}
In this section, we conduct experiments to answer the following research questions:
% \begin{itemize}[leftmargin=*]
% \textbf{RQ1:} Can MemoRec effectively model long-term user interests to improve recommendation quality?
% \textbf{RQ2:} Are the interactions retrieved by MemoRec more effective than random selections?
% \textbf{RQ3:} Can MemoRec utilize distant long-term histories for recommendations?
% \end{itemize}
\begin{itemize}[leftmargin=*]
\item \textbf{RQ1:} Can MemoRec effectively model long-term user interests to improve recommendation quality?
\item \textbf{RQ2:} Are the interactions retrieved by MemoRec more effective than random selections?
\item \textbf{RQ3:} Can MemoRec utilize distant long-term histories for recommendations?
\end{itemize}

% MemoRec是否可以有效地建模long-term interest以提升推荐质量呢
% MemoRec是否召回的历史交互相比随机选择的是否更有效呢
% MemoRec 是否可以建模较远的长期history呢
% verify the effectiveness of the MemoRec.
% answer the following research questions: \textbf{RQ1:} ?
% \textbf{RQ2:}



\subsection{Experimental Setup}
% -------------------------1211 tianhao
\noindent \textbf{Datasets.} We conduct experiments on two representative datasets from Amazon Product Reviews\footnote{\url{https://jmcauley.ucsd.edu/data/amazon/}.}: Amazon Book (Book) and Amazon Movie (Movie). These datasets contain user reviews from Amazon, collected from 1996 to 2018.
Due to the large scale of both Book and Movie, we extract data from 2017 for our experiments, allocating the first 10 months for training, and the remaining two halves for validation and testing, respectively.
We take the reviews as the interaction behaviors and sort the reviews from one user by time to form the behavior sequence.
We set the maximum behavior sequence length to 100, using the most recent 10 behaviors for the short-term sequential features and the rest as the long-term memory bank. To ensure data quality, we filter out items with fewer than 5 interactions and sequences shorter than 20 behaviors.

% We set the maximum behavior sequence length as 100, with the most recent 10 behaviors as the input of the short-term user sequential feature, and others as the long-term memory bank. To ensure data quality, we filter out infrequent items with fewer than 5 interactions.
% Additionally, as this work studies long-term user interest, we exclude sequences with lengths less than 20. 
% Additionally, we filter out infrequent items with fewer than 5 interactions to ensure data quality.


% As this work studies long-term user interest, we filter out users with fewer than 20 interactions. 
% Additionally, we filter out infrequent items with fewer than 5 interactions to ensure data quality.
% To evaluate the sequential recommendation, we use the 放在details


\noindent \textbf{Baselines.} We select three famous LLM-based methods as baselines, including 1) \textbf{BIGRec~\cite{bigrec}}, which is an LLM-based generative recommendation model that grounds the output of LLM to actual item space using an L2 distance;
2) \textbf{ReLLa~\cite{rella}}, which models long-term user interest in discriminative recommendations by semantically retrieving the most relevant interacted items to the target item. In generative recommendations, as the target item is unavailable, we adapt ReLLa by using the short-term user behaviors as the query for retrieving; 3) \textbf{TRSR~\cite{trsr}}, which extracts long-term user interest by  
first segmenting user historical behaviors and subsequently utilizing LLMs to summarize long-term user interest from the blocks. Additionally, we choose \textbf{SASRec~\cite{sasrec}}, a representative conventional method, as a baseline. SASRec employs a self-attention mechanism to capture sequential patterns.

% several representative methods as baselines, including 1) SASRec~\cite{sasrec}, which is a traditional sequential recommendation method that uses a self-attention mechanism to grasp sequential patterns; 
% 2) BIGRec~\cite{bigrec}, which is an LLM-based generative recommendation model that grounds the output of LLM to actual item space using an L2 distance;
% 3) ReLLa~\cite{rella}, which  models long-term user interest in discriminative recommendations by semantically retrieving the most relevant historical interactions to the target item. In generative recommendations, as the target item is unavailable, we adapt ReLLa by using the short-term item history as the query for retrieval; 4) TRSR~\cite{trsr}, which models long-term user interest by  
% first segmenting user historical behaviors and subsequently utilizing LLMs to summarize long-term user interest from . 

\noindent \textbf{Evaluation metrics.}
Following previous works~\cite{sasrec, bigrec}, we leverage the next-item recommendation scheme. 
To evaluate the top-K recommendation performance, we employ two widely adopted metrics: Recall, and Normalized Discounted Cumulative
Gain (NDCG). 


\noindent \textbf{Implementation details.}
We optimize SASRec and the retriever of MemoRec using BCE loss and the Adam optimizer, with learning rates searched in [1e-2, 1e-3, 1e-4] and batch sizes in [256, 512, 1,024, 2,048]. For LLM-based methods, we use Llama2-7B as the LLM backbone, optimizing with the AdamW optimizer and exploring learning rates in [1e-3, 1e-4, 1e-5] and setting the batch size to 32. For MemoRec, we optimize using the Adam optimizer with learning rates searched in [1e-1, 1e-2, 1e-3, 1e-4, 1e-5] and batch sizes in [512, 1,024, 2,048]. An early stopping strategy is applied based on Recall@1 on the validation set, with a patience of 10. 

% tuned the temperature coefficients of KL-loss in the range of [10, 1, 0.1, 0.01] and 
\begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.4}
\caption{The comparison between MemoRec and baselines.}
\label{table2} 
\begin{tabular}{lcccc}
\toprule
Dataset                & Model   & Recall@1 & Recall@5 & NDCG@5 \\
\hline
\multirow{5}{*}{Book}  & SASRec  & 0.0047   & 0.0214   & 0.0128 \\
                       & ReLLa   & 0.0045   & 0.0065   & 0.0055 \\
                       & TRSR    & \underline{0.0283}   & 0.0351   & 0.0319 \\
                       & BIGRec  & 0.0281   & \underline{0.0360}   & \underline{0.0323} \\ 
                       % \cline{2-5}
\rowcolor[HTML]{E9E9E9}                       & MemoRec & \textbf{0.0291}   & \textbf{0.0379}   & \textbf{0.0338} \\
\hline
\multirow{5}{*}{Movie} & SASRec  & 0.0329   & 0.0554   & 0.0437 \\
                       & ReLLa   & 0.0029   & 0.0050   & 0.0030  \\
                       & TRSR    & \underline{0.0591}   & \underline{0.0637}   & \underline{0.0613} \\
                       & BIGRec  & 0.0575   & 0.0616   & 0.0597 \\ 
                       % \cline{2-5}
\rowcolor[HTML]{E9E9E9}                       & MemoRec & \textbf{0.0601}   & \textbf{0.0638}   & \textbf{0.0621} \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Overall Results (RQ1)}

% ---------------------tianhao1211
Table~\ref{table2} illustrates the overall performance comparison between MemoRec and baselines, where we can find:

\begin{itemize}[leftmargin=*, itemsep=2pt, topsep=2pt, parsep=2pt]
    \item MemoRec achieves the best performance. Comparing MemoRec to BIGRec, MemoRec performs better, which verifies 1) the importance of modeling long-term history for generative LLM-based recommendations and 2) the effectiveness of our proposed memory-retrieval framework in modeling long-term interest.
    \item Comparing MemoRec and Rella, MemoRec demonstrates superior performance. This is because ReLLa's semantic retrieval can only recall information similar to the current interest, limiting its ability to provide useful signals for prediction. In contrast, MemoRec uses a learning-based approach to train the retriever, enabling it to extract beneficial information from history.
    \item TRSR outperforms BIGRec on Movie but performs similarly on Book.  We attribute this to the LLM's weaker language understanding of books compared to movies, limiting its ability to extract useful long-term interests from Book data. In contrast, MemoRec overcomes this limitation by leveraging a learning-based paradigm to retrieve effective information from memory.

    
    % This can be attributed to LLM's weaker language understanding of books compared to movies making it cannot extract useful long-term interest on Book, 
    % indicating the limitation of directly using LLM's summary to extract long-term interest. In contrast, MemoRec could effectively 不受语言理解能力的限制， 通过学习的范式从记忆中提取有效信息。
    
    
    % , suggesting that long-term effects in TRSR offer limited benefits for the book dataset. 
    
    % This may be because LLMs understand movies better, making it easier to extract user preferences from movie histories. In contrast, MemoRec effectively models long-term preferences through data-driven learning, overcoming LLM limitations.
\end{itemize}


% todo 阅读intro+分析+analysis

% 1）MEmorec取得最好结果。memorec比bigrec更好, a).强调加长历史的重要性, b).以及用学习方法建模长历史的有效性.
% 2) Memorec outperform rella, 说明用学习召回地相比语义召回更有效。
% 3) trsr outperform bigrec in movie，但在book上与bigrec类似，意味着trsr在book数据集上引入长期效应没有正面作用。这可能是由于LLM对movie对book的理解更好，更容易从movie的行为历史中提取用户偏好。这说明，用LLM提取long-term user preference的做法受到LLM语言理解能力的限制。相反，Memorec可以通过数据中关联的学习有效建模长期偏好。




% ------------------old-----------------

% \begin{itemize}[leftmargin=*]
%     \item    
%     MemoRec integrates a long-term interest retrieval model into BIGRec, resulting in significant improvements over the original BIGRec. Furthermore, when compared to existing LLM-based methods that utilize long-term interests such as ReLLa and TRSR, our method demonstrates a more effective approach. 
%     \item  ReLLa exhibits the poorest recommendation performance across all datasets and metrics. This is because ReLLa was designed for discriminative recommendation scenarios, and in generative recommendation scenarios, it can only use the semantic representation of local input information instead of the target item to retrieve long-term interests, which severely limits its performance. 
%     \item TRSR shows unstable performance across the two datasets. Specifically, on the Book dataset, the integration of long-term historical summaries with local input information leads to a performance loss (compared to BIGRec). This is due to the fact that summarizing a user's entire history into a single summarized text results in the loss of a large amount of long-term interest and heavily relies on the summarization capabilities of the LLM. 
    
% \end{itemize}



% In this section, we compare the overall performance of the proposed MemoRec with baselines. As shown in Table~\ref{table2}, MemoRec outperforms all baselines across both datasets in terms of the evaluation metrics Recall@1, Recall@5, and NDCG@5. 

% MemoRec integrates a long-term interest retrieval model into BIGRec, resulting in significant improvements over the original BIGRec. Furthermore, when compared to existing LLM-based methods that utilize long-term interests such as ReLLa and TRSR, our method demonstrates a more effective approach. 

% $\bullet$  ReLLa exhibits the poorest recommendation performance across all datasets and metrics. This is because ReLLa was designed for discriminative recommendation scenarios, and in generative recommendation scenarios, it can only use the semantic representation of  local input information instead of target item to retrieve long-term interests, which severely limits its performance. 

% $\bullet$  TRSR shows unstable performance across the two datasets. Specifically, on the Book dataset, the integration of long-term historical summaries with local input information leads to a performance loss (compared to BIGRec). This is due to the fact that summarizing a user's entire history into a single summarized text results in the loss of a large amount of long-term interests and heavily relies on the summarization capabilities of the LLM. 

% In conclusion, our proposed method can retrieve the long-term interests genuinely needed by the LLM in generative recommendation scenarios, thereby demonstrating an efficient and stable ability to recommend by integrating both long-term and short-term interests.


\subsection{Analysis}
\subsubsection{Comparison with Random Retrieval (RQ2).} 
% To validate the effectiveness of MemoRec, we compare its performance with random retrieval. 
We compare MemoRec with random retrieval and present the results in Figure~\ref{fig:wrand}, where we find MemoRec consistently outperforms random retrieval across both datasets. 
Notably, both the median and 25th percentile values of MemoRec exceed those of random retrieval across all metrics.
% Notably, the mediean percentile values of MemoRec exceed the median of random retrieval across all metrics. 
This improvement suggests that MemoRec effectively retrieves beneficial long-term history, enhancing future predictions.
% This improvement can be attributed to MemoRec's capability to effectively avoid retrieving irrelevant or harmful long-term interests, unlike random retrieval.
% To validate the effectiveness of MemoRec, we present a performance comparison with random retrieval. As shown in Figure~\ref{fig:wrand}, MemoRec outperforms random retrieval across both datasets, and its retrieval performance demonstrates robustness. Specifically, the median performance of MemoRec on all metrics, as well as its 25th percentile, is higher than the median of random retrieval. This improvement is attributed to MemoRec's ability to effectively avoid retrieving harmful long-term interest compared to random retrieval.


% \subsubsection{Key Factor of Retrieval.}
% Figure~\ref{fig:bm_timestamp} demonstrates that the effectiveness of MemoRec in enhancing recommendations is closely associated with the timing of user interactions. 
% On the movie dataset, MemoRec predominantly improves recommendations for interactions that occur within a shorter time interval from historical events. This suggests a latent user behavior pattern where users are often influenced by movies they have recently watched.
% In contrast, on the book dataset, books tend to have a more lasting impact on user interests. Consequently, MemoRec enhances recommendations for interactions that occur further away from historical events.





\subsubsection{Case Study (RQ3).}
% We randomly select some users who can
% We randomly select some users with Recall@1 improved after incorporating the long-term interaction histories retrieved by MemoRec, and analyze the interaction timestamps of long-term interests retrieved by MemoRec.
We analyze the timestamps of long-term histories retrieved by MemoRec for test samples whose Recall@1 improved after incorporating these histories in Figure~\ref{fig:case_study}. 
% We analyze the interaction timestamps of long-term interests retrieved by MemoRec for samples where local information alone failed, but incorporating long-term histories successfully retrieved the next item, as shown in Figure~\ref{fig:case_study}.
The figure shows that MemoRec can retrieve users' long-term behaviors even from distant past interactions, highlighting its capability to effectively capture long-term user interests.

% Figure~\ref{fig:case_study} presents the results, showing that MemoRec successfully retrieves users' long-term behaviors even from distant past interactions. 
% This emphasizes MemoRec's capability to capture  
% user's long-term interests.






 
% This highlights its potential for building lifelong generative recommendation systems powered by LLMs.


% 分两段。


% For SASRec and the retriever of MemoRec, we optimize the parameters with BCE loss and the Adam optimizer. We search the learning rate in 
% [1e-2, 1e-3, 1e-4] and batch size in [256, 512, 1,024, 2,048]. For LLM-based methods, we employ Llama2-7B as the LLM backbone and optimize them with the AdamW optimizer. We adjust the learning rate in 
% [1e-2, 1e-3, 1e-4] and batch size in [256, 512, 1,024, 2,048]. For the MemoRec, we search the temperature coefficient in the range of [10, 1, 0.1, 0.01]. We adopt a early stopping strategy based the Recall@1 on validation set with the patience of 10. 
% To ensure a fair comparison, the 
% Our proposed method and the baselines involve both 
% To ensure a fair comparison, the input



% We conduct experiments on two representative datasets: Amazon Book (Book) and Amazon Movie (Movie).





% \subsubsection{Datasets}
% %我们从两个广泛使用的真实数据集做实验 Amazon book and movies。这两个数据集都含有大量长期用户，有助于我们验证我们方法结合长短期兴趣的能力。我们抽取2017年的数据作为实验数据集，且将10月之前的数据作为训练集，11和12月的数据作为验证和测试。为了公平比较（不增加额外的数据），我们指定为训练集为能够获得的长期兴趣记忆库，即检索的对象仅限于在训练集中检索。在训练集中我们将交互次数少于5的不热门的用户和商品过滤掉，同时过滤掉验证和测试集中在记忆库中交互次数多于20次，少于100次的用户，保证我们测试的对象是长期用户。同时将过滤后的11和12月份数据按照时间顺序1:1划分为验证集和测试集。此外，按照我们保留最后 10 次交互作为历史序列用于训练生成式推荐模型，在本文中，该历史序列被称为短期上下文（兴趣）。
% We conduct experiments using two widely adopted real-world datasets, Amazon Books (Book) and Amazon Movies (Movie). These datasets contain a significant number of long-term users, which allows us to evaluate the capability of our method to integrate long- and short-term interests effectively.  

% We extracted data from 2017 for our experiments, using data prior to October as the training set, while data from November and December served as the validation and test sets. To ensure a fair comparison (without introducing additional data), we designated the training set as the only available long-term interest memory bank, meaning retrieval was restricted to items present in the training set.  

% In the training set, we filtered out infrequent users and items with fewer than five interactions. Additionally, we excluded users in the validation and test sets who had more than 20 or fewer than 100 interactions in the memory bank to ensure that the evaluation focused on long-term users. The filtered data from November and December was then split 1:1 in chronological order into the validation and test sets.  

% Following standard practices, we retained the last 10 interactions as the historical sequence for training and testing the generative recommendation models (baselines). In this work, this historical sequence is referred to as the short-term context (interest).



% \subsubsection{backbone and Baselines}
% %我们选择了一个最常见的传统模型SASRec以及两个最新的专注于LLM场景下建模长期用户兴趣的方法：1）R e L L a：在LLM判别式推荐场景下，ReLLa通过目标商品的语义信息，对用户的历史交互商品进行召回，通过将由时间近邻的构造的指令替换为语义近邻来判断目标商品是否值得被推荐。然而在生成式推荐场景下，目标商品是无法获得的，故而我们在本文中，通过短期交互历史作为替代做语义检索。2）TRSR：该方法通过LLM的总结能力，对用户的所有交互历史生成总结文本，然后将用户的总结和用户的短期兴趣构建为指令，微调LLM。
% We select state-of-the-art LLM-based generative recommendation model BIGRec as our backbone. BIGRec performs recommendation in two stages: First, it generates tokens based on instructions constructed from the user's short-term context. Then, it maps the LLM embeddings of these tokens to existing items in the dataset using L2 distance.

% In addition to BIGRec, we also selected three baselines including one of the most common traditional models, SASRec~\cite{sasrec}, and two state-of-the-art methods focused on modeling long-term user interests in LLM-based recommendation scenarios: 1) ReLLa~\cite{rella}: In the discriminative recommendation setting with LLMs, ReLLa retrieves the user’s interaction items in memory based on the semantic information of the target item. It replaces time-based neighbors in instructions with semantically similar neighbors to determine whether the target item is worth recommending. However, in the generative recommendation setting, the target item is not available. Therefore, in this work, we adapt ReLLa by using short-term interaction history as a substitute for semantic retrieval. 2) TRSR~\cite{trsr}: This method leverages the summarization capabilities of LLMs to generate a summary of the user’s preferences of all interaction items in memory. It then combines the user's summary with their short-term context to construct an instruction for fine-tuning the LLM.  


% \subsubsection{Metrics}
% We use two commonly used metrics, Recall and NDCG as the evaluation metrics.
% To evaluate the model’s top-K recommendation performance, we use two commonly used
% metrics: Recall@K and NDCG@K, which we compute in the all-ranking evaluation setting. In this paper, we set K as 1 and 5. 
% \subsubsection{Implementation details}
% For the SASRec, we conduct a grid search for learning rate and weight decay searched in [1e-2, 1e-3, 1e-4] and batch size within the range of [256,512,1024,2048]. The model is optimized by using BCE loss and the Adam optimizer. For LLM-based methods (BIGRec, \zjz{ReLLa}, TRSR), we apply Llama2-7B as the LLM backbone. we use the AdamW optimizer and adjust the learning rate within the range of [1e-3, 1e-4, 5e-5]. During the training, we adjust the learning rate over steps using a cosine scheduler and set the early stop strategy based on Recall@1 metric. For training retriever, we adopted the same experimental setting with SASRec including search range of the learning rate, weight decay, batch size and the Adam optimizer. We also search the temperature coefficient in KL-loss within the range of [10, 1, 0.1, 0.01]. All experiments were conducted on an \zjz{NVIDIA A100 GPU}.

% \subsection{Comparison with State-of-the-arts}
% \subsection{Results}





% 在这个章节里，我们比较了提出的MemoRec和baselines的整体性能。正如表2中展示的，MemoRec在两个数据集的测评指标Recall@1， Recall@5 ，NDCG@5上超越了所有的baselines。该方法为BIGRec配备的长期兴趣检索模型，引入了长期兴趣，在BIGRec的基础上得到了明显的增益。更多地，比较当前存在的基于LLM的利用长期兴趣的方法（ReLLa，TRSR），我们的方法是一种更高效的方式。值得注意的是，ReLLa在所有数据和指标上，均表现出较差的推荐性能，这是因为ReLLa是在判别式推荐场景下提出的，而在生成式推荐场景下，仅仅能够使用短期兴趣的语义表示代替目标商品对长期兴趣检索，严重限制了ReLLa的性能。TRSR在两个数据集上表现出了不稳定的性能，在Book数据集上，以长期兴趣的总结与短期兴趣融合导致了性能的损失（对比BIGRec），这是由于长期兴趣的总结会丢失大量的用长期兴趣，而且十分依赖LLM的总结能力。综上所述，我们提出的方法，在基于LLM的生成式推荐场景下，能够检索到LLM真正需要的长期兴趣，故而展现出了高效且稳定的融合长短期兴趣做推荐的能力。
% \subsection{Overall performance comparison.}

% In this section, we compare the overall performance of the proposed MemoRec with baselines. As shown in Table~\ref{table2}, MemoRec outperforms all baselines across both datasets in terms of the evaluation metrics Recall@1, Recall@5, and NDCG@5. 

% MemoRec integrates a long-term interest retrieval model into BIGRec, resulting in significant improvements over the original BIGRec. Furthermore, when compared to existing LLM-based methods that utilize long-term interests such as ReLLa and TRSR, our method demonstrates a more effective approach. 

% $\bullet$  ReLLa exhibits the poorest recommendation performance across all datasets and metrics. This is because ReLLa was designed for discriminative recommendation scenarios, and in generative recommendation scenarios, it can only use the semantic representation of  local input information instead of target item to retrieve long-term interests, which severely limits its performance. 

% $\bullet$  TRSR shows unstable performance across the two datasets. Specifically, on the Book dataset, the integration of long-term historical summaries with local input information leads to a performance loss (compared to BIGRec). This is due to the fact that summarizing a user's entire history into a single summarized text results in the loss of a large amount of long-term interests and heavily relies on the summarization capabilities of the LLM. 

% In conclusion, our proposed method can retrieve the long-term interests genuinely needed by the LLM in generative recommendation scenarios, thereby demonstrating an efficient and stable ability to recommend by integrating both long-term and short-term interests.

% \subsection{Analysis}
\begin{figure}[tbp]
  \centering            
  \subfloat{
        \label{fig:book_wrand}\includegraphics[width=0.225\textwidth]{Fig/b_wrand.pdf}}
   \subfloat{
        \label{fig:movie_wrand}\includegraphics[width=0.225\textwidth]{Fig/m_wrand.pdf}} 
  % \caption{The timestamps of user's next interaction for augmentable and non-augmentable users.}
  \caption{Performance comparison of MemoRec and random retrieval. The bottom, middle, and top lines of the box represent the 25th percentile, median (50th percentile), and 75th percentile, respectively.}
  % hit@1原来不能命中的，现在命中了，标题尽量概括全，正文就不重复。
  \label{fig:wrand}
\end{figure}

\begin{figure}[tbp]
  \centering            
  \subfloat{
        \label{fig:case_study_book}\includegraphics[width=0.225\textwidth]{Fig/case_study_book.pdf}}
  \subfloat{
        \label{fig:case_study_movie}\includegraphics[width=0.225\textwidth]{Fig/case_study_movie.pdf}}
  \caption{
%   (a) 
%    Timestamps of test samples, where "True" denotes samples where local information fails but with long-term history successfully retrieve the next item (MemoRec improves Recall@1), and "False" denotes samples where 
% where local information fails, and incorporating long-term history also fails to retrieve the next item.
%   (b) 
% Historical interaction time of some samples where incorporating long-term history improves Recall@1. 
Visualization of the historical interaction times for some samples where incorporating long-term history improves Recall@1.
The yellow circles represent the long-term history retrieved by MemoRec.
  % Timestamps of retrieved long-term history for cases where incorporating long-term history leads to improvements in Recall@1.
  % Timestamps of retrieved long-term history for some cases where incorporating long-term history improves Recall@1.
  % Interaction timestamps of long-term history retrieved by MemoRec for cases where Recall@1 improved after incorporating the long-term history.
  % Distribution of the timestamp of test samples, where "True" indicates interactions where local information fails but incorporating long-term interests successfully retrieves next item (MemoRec improves Recall@1), and "False" indicates interactions where both local and long-term information fails to retrieve next item.
  % where the x-axis labels indicate: "True" – interactions where local information alone fails, but incorporating long-term 
% interest successfully retrieves user interests (MemoRec improves Recall@1), and "False" – interactions where both local information and long-term history fail to retrieve user interests.
  % The timestamps of user's interaction at test time for augmentable and non-augmentable users. "True" means the MemoRec can enhance the recommendation for this interaction of the user.  
  % (b) Case study: the interaction times of the user's relevant long-term interests which is obtained by MemoRec.
  }
  \label{fig:case_study}
\end{figure}


% 消融实验
% 
% \subsubsection{Ablation study of retriever.}
% % 为了验证我们检索器的有效性，我们展示了我们训练得到的检索器和随机检索的性能比较。如图1，MemoRec在两个数据集均比随机检索高且性能的提升具有鲁棒性。具体地，MemoRec在所有指标上的中位数均比随机检索高。不仅如此，其25 百分位数均高于随机检索的中位数，这是由于MemoRec相对于随机检索能够有效避免检索到有害的内容。
% % To evaluate the effectiveness of our retriever, we present a performance comparison between our MemoRec and random retrieval. As shown in Figure 1, MemoRec consistently outperforms random retrieval across both datasets, demonstrating robust performance improvements. Specifically, the median performance of MemoRec on all metrics is higher than that of random retrieval. Furthermore, the 25th percentile of MemoRec's performance surpasses the median of random retrieval. This is attributed to MemoRec's ability to effectively avoid retrieving harmful content compared to random retrieval.

% To validate the effectiveness of MemoRec, we present a performance comparison with random retrieval. As shown in Figure~\ref{fig:wrand}, MemoRec outperforms random retrieval across both datasets, and its retrieval performance demonstrates robustness. Specifically, the median performance of MemoRec on all metrics, as well as its 25th percentile, is higher than the median of random retrieval. This improvement is attributed to MemoRec's ability to effectively avoid retrieving harmful long-term interest compared to random retrieval.

% \subsubsection{Key factor of retrieval.}
% 我们发现MemoRec能否增强推荐与用户的交互时间这一关键因素有关。MemoRec有潜力根据在数据集上用户表现出来的与交互时间相关的潜在行为模式进行检索，并增强推荐。如图1，根据能否被MemoRec检索增强分为的2组用户交互之间存在很明显的交互时间差异。在movie数据集上，MemoRec能为与历史时间相距不太远的交互行为进行检索增强推荐，这可能是因为该数据集包含一个潜在的用户行为模式，即用户一般在短期内会被刚看完的一场电影所影响，。而在book数据集的书籍更倾向于对用户兴趣的长期影响，故而MemoRec能增强与历史交互时间相距较远的交互。同时，该现象能够进一步加强table1中的结论，即不像trsr，MemoRec能够根据不同数据集中用户的潜在行为模式提供稳定的增强效果。
% Figure~\ref{fig:bm_timestamp} illustrates that whether MemoRec can enhance recommendations is closely related to the time of user interaction, and the time of interactions which can be enhanced focused on a . As Figure~\ref{fig:bm_timestamp} shows, there is a significant difference in interaction time between the two groups of users, categorized based on whether their interactions can be enhanced by MemoRec. 

% In the Movie dataset, MemoRec is capable of enhancing recommendations for interactions that occurred relatively close in time to interactions in memory. This may be due to the fact that the movie dataset involves an underlying pattern of user behavior, i.e., users are generally influenced by recently watched movies over a short period. In contrast, in the Book dataset, books may tend to have a more long-term influence on user interests. As a result, MemoRec is able to enhance interactions that are further removed from interaction times in memory.

% 图~ref{fig:bm_timestamp}说明，MemoRec 能否增强推荐效果与用户交互的时间密切相关，且能被增强的用户交互主要发生在特定的时间范围内，我们将其称作增强时间区间。增强时间区间存在并且会随着数据集变化，一个可能的原因是由于数据集中商品的特点，用户受到长期兴趣的影响的时间范围不同，而memorec能够有效的捕捉到该时间范围做增强推荐。
% 增强时间间隔存在并且会随着数据集变化，一个可能的原因是由于数据集中的项目的特性和差异性，这会导致该数据平台上用户在特定的时间范围内会显著地受到长期兴趣的影响。



% Figure~\ref{fig:bm_timestamp} demonstrates that the effectiveness of MemoRec in enhancing recommendations is closely associated with the timing of user interactions. Specifically, user interactions that can be enhanced predominantly occur within a specific time range, which we refer to as the enhancement time interval. 
% The presence of the enhancement time interval, as well as its variation across datasets, may be attributed to the characteristics of the items within the datasets, which may lead to users on this data platform being significantly influenced by long-term interests within a specific time range.
% MemoRec is capable of effectively capturing this time range to perform enhanced recommendations.

% This observation further reinforces the conclusion in Table~\ref{table2}: unlike TRSR, MemoRec provides stable augmentation effects by capturing enhancement time intervals across different datasets.

% \subsubsection{Case study.}
% % 我们通过图1展示了用户被检索的相关长期兴趣的交互时间。图中，MemoRec能够成功检索时间上很久远的用户长期兴趣，这也为用户终身推荐系统的构建提供了可能。
% Figure~\ref{fig:case_study} is a case study showing the interaction times of user's relevant long-term interests retrieved by MemoRec.
% This figure shows that MemoRec successfully retrieves users' long-term interests even from distant past interactions, which opens up possibilities for building lifelong generative recommendation powered by LLM.










































% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/case_study.pdf}
%   \caption{% 用户的长期兴趣以及MemoRec检索到的该用户相关长期兴趣的出现时间。
%   Case study: The timestamps of user's long-term interests and the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}





% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/movie_posi_his_time_user.pdf}
%   \caption{
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}


% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/bm_time_rand.pdf}
%   \caption{
%   The timestamps of the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}



% \begin{figure*}[tbp]
%   \centering            
%   \subfloat[local-time]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.33\textwidth]{Fig/compare_wrand.pdf}}
%   \subfloat[local-time-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.33\textwidth]{Fig/bm_local_time.pdf}}
%   \subfloat[local-time-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.33\textwidth]{Fig/case_study.pdf}}
%   \caption{The timestamps of user's next interaction for augmentable and non-augmentable users.}
%   \label{fig:DNS}
% \end{figure*}

% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/compare_wrand.pdf}
%   \caption{
%   The retrieval capability of MemoRec compared to random retrieval.
%   }
%   \label{}
% \end{figure}




% \begin{table}[]
% % \centering
% \caption{The statistics of datasets.}
% \begin{tabular}{ccccc}
% \hline
% Dataset &$\#$Users    &$\#$Items    &train  &test   \\
% \midrule
% Book      &15,400 &1,000 &311,704 &48,600 \\
% Movie     &1411 &3327 &1,934,404 &2,742,166 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[tbp]
%   \centering            
%   \subfloat[his-len]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.25\textwidth]{Fig/bm_his_len.pdf}}
%   \subfloat[his-len-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.25\textwidth]{Fig/bm_his_len_rand.pdf}}
%   \caption{% 能够被增强的用户和不能被增强的用户的历史兴趣长度
%   Historical length of interest for users who can be augmented and users who cannot be augmented.
%   }
%   \label{fig:DNS}
% \end{figure}

% \begin{figure}[tbp]
%   \centering            
%   \subfloat[local-rank-len]{
%         \label{fig:DNS_yahoo}\includegraphics[width=0.25\textwidth]{Fig/bm_local_rank.pdf}}
%   \subfloat[local-rank-rand]{
%         \label{fig:DNS_kuairec}\includegraphics[width=0.25\textwidth]{Fig/bm_local_rank_rand.pdf}}
%   \caption{
%   The recommendation capabilities of short-term contexts for augmentable and non-augmentable users.
%   }
%   \label{fig:DNS}
% \end{figure}

% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=\linewidth]{Fig/book_posi_his_time_user.pdf}
%   \caption{% 用户的长期兴趣以及MemoRec检索到的该用户相关长期兴趣的出现时间。
%   Case study: The timestamps of user's long-term interests and the relevant long-term interests retrieved by MemoRec.
%   }
%   \label{}
%   % \vspace{-10pt}
% \end{figure}



